FLEXIS: FLEXible Frequent Subgraph Mining using Maximal Independent Sets

Frequent Subgraph Mining (FSM) is the process of identifying common subgraph patterns that surpass a predefined frequency threshold. While FSM is widely applicable in fields like bioinformatics, chemical analysis, and social network anomaly detection, its execution remains time-consuming and complex. This complexity stems from the need to recognize high-frequency subgraphs and ascertain if they exceed the set threshold. Current approaches to identifying these patterns often rely on edge or vertex extension methods. However, these strategies can introduce redundancies and cause increased latency. To address these challenges, this paper introduces a novel approach for identifying potential k-vertex patterns by combining two frequently observed (k - 1)-vertex patterns. This method optimizes the breadth-]first search, which allows for quicker search termination based on vertices count and support value. Another challenge in FSM is the validation of the presumed pattern against a specific threshold. Existing metrics, such as Maximum Independent Set (MIS) and Minimum Node Image (MNI), either demand significant computational time or risk overestimating pattern counts. Our innovative approach aligns with the MIS and identifies independent subgraphs. Through the "Maximal Independent Set" metric, this paper offers an efficient solution that minimizes latency and provides users with control over pattern overlap. Through extensive experimentation, our proposed method achieves an average of 10.58x speedup when compared to GraMi and an average 3x speedup when compared to T-FSM

==> algorithms/differentTopology.tex <==
\begin{algorithmic}[1]
  \Require{CoreGraph $cg$, generator $gen$, marked vertex topology $topo$}
  \Ensure{bool}
  \Procedure{differentTopology}{\textit{cg, gen, topo}}
  \State $\text{topo}^{b} \gets \Call{space}{cg.C_n^{u_m}, topo, \textbf{C}}$ \label{alg:line:space_canon}
  \State $\text{topo}^{g} \gets \Call{permute}{cg.B_n^{u_m}, gen, \text{topo}^{b}}$ \label{alg:line:permute}
  \State $\text{topo}^{new} \gets \Call{space}{cg.B_n^{u_m}, \text{topo}^{g}, \textbf{I}}$ \label{alg:line:space_canon_inverse}
  \State \Return $\text{topo}^{new} \neq topo$ \label{alg:line:dt:return}
  \EndProcedure
\end{algorithmic}


==> algorithms/findAllMatching.tex <==
\begin{algorithmic}[1]
  \Require {VFState $s$}
  \Ensure {VFState $s.count$}
  \Procedure{FindAllMatchings}{$s$}
    \State $n_1 \gets \emptyset$
    \State $n_2 \gets \emptyset$
    \State $cF \gets \False$~\label{line:findAllMatching:cf1}
    \sWhile { $s.\FunctionCall{NextPair}{n_1, n_2}$ } {
      \sIf { $\Not{} s.\FunctionCall{MiningPossible}{n_1, n_2}$ } { \Continue }
      \sIf { $\Not{} s.\FunctionCall{IsFeasible}{n_1, n_2}$ } { \Continue }
      \State $s1 \gets s$
      \State $s1.\FunctionCall{AddPair}{n_1, n_2}$
      \sIf { \FunctionCall{FindAllMatchingsRec}{$s1, cF$} } {
        \Return \True
      }
      \State $cF \gets \False$~\label{line:findAllMatching:cf2}
    }
    \State \Return \False
  \EndProcedure
  \Require {VFState $s$, Boolean $cF$ (passed by reference)}
  \Ensure {VFState $s.count$, find more matchings}
  \Procedure{FindAllMatchingsRec}{$s, cF$}
  \sIf { s.\FunctionCall{IsGoal}{} } {
    \State $cF \gets \True$~\label{line:findAllMatchingRec:cf3}
    \State \Return $\FunctionCall{visitor}{s}$
  }
  \sIf { s.\FunctionCall{IsDead}{} } {
    \State \Return $\False$
  }
  \State $n_1 \gets \emptyset$
  \State $n_2 \gets \emptyset$
  \sWhile { $s.\FunctionCall{NextPair}{n_1, n_2}$ } {
    \sIf { $\Not{} s.\FunctionCall{MiningPossible}{n_1, n_2}$ } { \Continue }
    \sIf { $\Not{} s.\FunctionCall{IsFeasible}{n_1, n_2}$ } { \Continue }
    \State $s1 \gets s$
    \State $s1.\FunctionCall{AddPair}{n_1, n_2}$
    \sIf { $\FunctionCall{FindAllMatchingsRec}{s1, cF}$ } {
      $\Return \True$
    }
    \sIf { $cF$ } { \Return \False }~\label{line:findAllMatchingRec:cf4}
  }
  \State \Return \False
  \EndProcedure
\end{algorithmic}


==> algorithms/generateCoreGraph.tex <==
\begin{algorithmic}[1]
  \Require {$P$}
  \Ensure {$\FunctionCall{set}{c}$}
  \Procedure{generateCoreGraph}{$p$}
  \State $c \gets \emptyset$
  \sForAll{$\nu \in V(P)$} { \Comment{$\nu$ is marked vertex}
    \State $c \gets c \cup \FunctionCall{CoreGraph}{P, \nu}$ \Comment{disconnects $\nu$ from $P$}
  }
  \Return $c$
  \EndProcedure
\end{algorithmic}


==> algorithms/generateNewCliques.tex <==
\begin{algorithmic}[1]
    \Require {intermediates from algorithm~\ref{alg:generate:New:Patterns:nonclique}}
    \Ensure {Cliques with size $k$}
    \Function{generateNewCliques}{}
        \sIf{ $i \OR j \notin $ cliques } { \label{alg:line:cl:cliques}
            \State \Return
        }
        \State $mv \gets i.\Call{otherVertex}{}$ \label{alg:line:cl:otherV}
        \State $cliqBase \gets coreMap[i.parent()][mv]$ \label{alg:line:cl:cliqBase}
        \sForAll{ $[\_, c3] \in cliqueGroup$ }{
            \State $auto2s \gets c3.\Call{findAutomorphism}{{}}$ \label{alg:line:cl:fa}
            \sForAll{ $a2 \in auto2s$ } {
            \State $pc \gets i.\Call{mergeClique}{j, auto, mv, cliqBase, c3, a2}$~\label{alg:line:cl:merge}
            \sIf { $pc$ }{
                \State $P_{k+1}.\Call{add}{pc}$ \label{alg:line:cl:add}
            }
            }
        }
    \EndFunction
\end{algorithmic}


==> algorithms/generateNewPatterns.tex <==
\begin{algorithmic}[1]
  \Require {Set of size-$(k-1)$ pattern graphs $P^{(k-1)}$}
  \Ensure {Set of size-$k$ pattern graphs $P^{k}$}
  \Function{generateNewPatterns}{$ P^{(k-1)} $}
  \State  {\em coreGroups} $\gets \FunctionCall{CoreGroup}{P^{(k-1)}} $ \label{alg:gen:nc:cg:gen}
    \State $ P^k \gets \emptyset $
    \sForAll{ $cgID \in$ {\em coreGroups} }{ \label{alg:gen:nc:cg:iter1}
      \sForAll{$[C_i, C_j] \in \Call{pairs}{cgID}$}{ \label{alg:gen:nc:cg:iter2}
        \State $\text{autoList} \gets \Call{findAutomorphism}{cgID}$ \label{alg:gen:nc:fa}
        \sForAll{ $\alpha \gets \text{autoList} $ } {
          \State $\text{P} \gets \Call{merge}{C_i, C_j, \alpha} $ \label{alg:gen:nc:ma}
          \State $P^k.\Call{add}{P}$
          \State $P^k \gets P^k \cup \Call{generateNewCliques}{}$ \label{alg:gen:nc:gnc}
        }
      }
    }
    \State \Return $P^k$
  \EndFunction
\end{algorithmic}


==> algorithms/merge.tex <==
\begin{algorithmic}[1]
  \Require {CoreGraph cg1, cg2, permutation perm}
  \Ensure {PatternGraph np}
  \Procedure{merge}{\textit{cg1, cg2, perm}}
  \State {$np \gets$ attach marked vertex to cg1} \label{algo:line:cg:marked}
  \State {$cgm \gets $ cg2's marked label} \label{algo:line:other:marked}
  \State {$np \gets $ apply perm to np} \label{algo:line:merge:perm}
  \State {$np \gets $ addEdges from np to cgm} \label{algo:line:other:addedge}
  % \sForAll{ $topo \in cg2.topo$ } {
  %   \State $w_{new}^o \gets cg2.canon[cg2.topo]$~\label{algo:merge:line:canon}
  %   \State $w_{alt}^o \gets perm[w_{new}^o]$~\label{algo:merge:line:perm}
  %   \State $w_{new} \gets cg1.ci[w_{alt}^o]$~\label{algo:merge:line:inverse}
  %   \State $np.\Call{addEdge}{w_{new}, cg2.marked}$ \label{algo:line:other:addedge}
  % }
  \State \Return $np$
  \EndProcedure
\end{algorithmic}


==> algorithms/mergeNonClique.tex <==
\begin{algorithmic}[1]
  \Require {coreGroups:} \text{map of graph struct. \& core graph objs}
  \Ensure {newPatterns:} \text{list of merged patterns}
  \Procedure{generateNewPatterns}{\textit{coreGroups}}
  \sForAll{ $[k, cg] \in coregroups$ } {
    \sForAll{ $iiter \in \Call{iter}{cg, 0} $ } { \Comment \textit{iterator of cg from 0th pos}
      \sForAll{ $jiter \in \Call{iter}{cg, iiter}$ } {
        \State $\text{autos} \gets k.\Call{findAutomorphism}{\{iiter, jiter\}} $
        \sForAll{ $\text{auto} \gets \text{autos} $ } {
          \State $\text{p} \gets iiter.\Call{mergeAuto}{jiter, auto} $
          \State $newPatterns.\Call{add}{p}$
        }
      }
    }
  }
  \EndProcedure
\end{algorithmic}


==> algorithms/visitor.tex <==
\begin{algorithmic}[1]
  \Require {VFState $s$}
  \Ensure {boolean}
  \Procedure{visitor}{$s$}
    \State $s$.count $\gets$ $s$.count + 1
    \sForAll { $\nu \in s.v_d$ } {
      \State $s$.used[$\nu$] $\gets$ \True
    }
    \State \Return $s$.count >= $s$.threshold
  \EndProcedure
\end{algorithmic}


==> contents/abstract.tex <==
\begin{abstract}
  Frequent Subgraph Mining (FSM) is the process of identifying common subgraph patterns that surpass a predefined frequency threshold. While FSM is widely applicable in fields like bioinformatics, chemical analysis, and social network anomaly detection, its execution remains time-consuming and complex. This complexity stems from the need to recognize high-frequency subgraphs and ascertain if they exceed the set threshold. Current approaches to identify these patterns often rely on edge or vertex extension methods. However, these strategies can introduce redundancies and cause increased latency. To address these challenges, this paper introduces a novel approach for identifying potential $k$-vertex patterns by combining two frequently observed $(k-1)$-vertex patterns. This method optimizes the breadth-first-search, which allows for quicker search termination based on vertices count and support value. Another challenge in FSM is the validation of the presumed pattern against a specific threshold. Existing metrics, such as Maximum Independent Set (MIS) and Minimum Node Image (MNI), either demand significant computational time or risk overestimating pattern counts. Our innovative approach aligns with the MIS and identifies independent subgraphs. Through the \qoutes{Maximal Independent Set} metric, this paper offers an efficient solution that minimizes latency and provides users with control over pattern overlap. Through extensive experimentation, our proposed method achieves an average of 10.58x speedup when compared to GraMi and an average 3x speedup when compared to T-FSM.
\end{abstract}


==> contents/all.tex <==
%!TEX root = paper.tex

\newif\ifACM
\ifdefined\ACMformat
    \ACMtrue
\else
    \ACMfalse
\fi

\section{Introduction}~\label{sec:Introduction}
\ac{fsm} has gained significant attention in the past few years. FSM is defined as the identification of recurring subgraph patterns that occur more frequently than a predefined threshold. FSM finds extensive application within domains such as chemical information analysis~\cite{kong:2022:molecule}, bioinformatics~\cite{mrzic:2018:grasping}, anomaly detection in social networks~\cite{bindu:2016:mining}, and the detection of android malware~\cite{martinelli:2013:classifying}. In the context of bioinformatics and chemical information analysis, these derived subgraphs are employed to find patterns that facilitate protein prediction and molecule generation. In the context of social networking and android malware detection, the identification of frequent patterns plays an important role in determining deviations from expected behavioral norms, be it within applications or users~\cite{martinelli:2013:classifying}.

Despite the attention that the problem has received in the past few years, solving FSM still takes a lot of time. This complexity arises from the nature of the problem that requires determining if the frequency of a certain subgraph in a larger graph occurs over a certain threshold (support) - an NP-Complete problem.  This problem is generally solved in two steps, namely, 
\begin{enumerate*}
  \item the identification of potential high-frequency subgraphs within the large graph, and
  \item determination whether these subgraphs occur more than a predefined threshold.
\end{enumerate*}
Thus, to effectively solve the problem, determining an efficient method for both steps is important.

Considerable research efforts have been directed towards both steps of this approach. Step 1 has been tackled using techniques based on edge extension or vertex extension. In case of edge extension methods there are two main approaches. In the first approach, a possible $k$ edge subgraph is derived from two frequent $(k-1)$-subgraphs. The process of merging two viable subgraphs sharing identical $(k-2)$ edge subgraphs is detailed in multiple works~\cite{kuramochi:2004:efficient, kuramochi:2005:finding}. In the paper~\cite{kuramochi:2004:efficient}, transactional algorithms are employed. Here, a pattern is considered frequent if it appears in more than a specified number of distinct data graphs. However, it's essential to note that our paper diverges from this focus, as we consider a single graph mining, in which a pattern is considered frequent if it occurs over a certain number of times in a single data graph.
In the subsequent work~\cite{kuramochi:2005:finding}, a similar concept is proposed for single graphs. The second approach involves the addition of an edge to all frequent $(k-1)$-subgraphs followed by eliminating redundancies~\cite{yuan:2023:tfsm, elseidy:2014:grami}. Conversely, in the domain of vertex extension methods as illustrated by works such as~\cite{chen:2020:pangolin, chen:2022:efficient, yao:2020:locality, chen:2021:sandslash}, the potential $k$-vertex subgraphs are established by exhaustively generating all feasible extensions of $(k-1)$-vertex frequent subgraphs, and eliminating redundancies.

In case of vertex and edge extension methods based on adding a vertex/edge, the generation of possible patterns often introduces redundancies, leading to an undesirable increase in latency. A potential alternative to mitigate this issue is presented in~\cite{kuramochi:2005:finding}. However, this alternative method, which places emphasis on edges, results in graphs with the same number of vertices being positioned at different levels within the breadth-first-search exploration space. Consequently, the delayed occurrence of early termination criteria based on the number of vertices and support value contributes to increase in latency.

Thus, we propose a novel approach aimed at determining possible $k$-vertex patterns, which involves the synthesis of two frequently occurring $(k-1)$-vertex patterns. Notably, our method shares advantageous features with the approach detailed in~\cite{kuramochi:2005:finding}, particularly when compared to other vertex or edge extension methods. Additionally, our approach yields potential frequent graphs with an identical number of vertices situated at the same level during breadth-first-search. This unique attribute enables early termination of the search based on the number of vertices and support value, thereby minimizing latency.

Step 2 (verifying whether the presumed pattern meets a specific threshold) has also seen notable contributions. One widely recognized metric in this context is the \ac{mis}. This metric determines the frequency of a pattern by determining the count of disjoint, independent patterns that exist in the data graph. While this method is known for its precision, it is affected by its NP-Complete nature, consequently demanding substantial computational time for completion. An alternative strategy frequently employed is the \ac{mni}, which establishes the highest count of independent sets achievable for a given pattern within the original graph. Notably, this approach may yield non-disjoint independent sets, leading to vertex overlap among these sets. 

Although this method is fast, it has the potential to overestimate the count of patterns. Another method, that builds on \ac{mni}, known as fractional-score~\cite{yuan:2023:tfsm} has also been proposed which alleviates the overestimation problem, by introducing a contribution factor that determines how much each vertex can contribute to a certain pattern. Even though there is a reduction in the number of false positives, it still encounters a significant number of them. Both existing methods lack the option for users to control the intersection between the frequent patterns identified by using \ac{mni} and MIS (overlap). 

In contrast, our proposed approach introduces a mechanism to align with the MIS, which exclusively identifies independent patterns without vertex overlap. This is achieved through the utilization of \ac{mal}. \ac{mal} is an approximation on MIS. We leverage a mathematical relationship that exists between these metrics, which enables us to establish the lower bound of support for the \ac{mal} metric, based on the support for the MIS metric. The upper bound corresponds to the support value for MIS. Users can define the degree of overlap with the MIS metric by selecting the interpolation level, referred to as the \textit{slider value}. This way, they have control over the extent of overlap with the MIS metric, offering a metric applicable across various applications.

This paper makes the following contributions,

\begin{itemize}
  \item Propose a metric based on \qoutes{Maximal Independent Set}, that enumerates the occurrences of pattern graphs within a data graph.
  \item Develop the theoretical basis for merging subgraphs that guarantees potentially frequent patterns not being missed.
  \item Describe a technique to join two smaller yet frequently occurring subgraphs, each with $(k-1)$-vertices, thereby determining a potential subgraph with $k$-vertices.
  \item We implemented the algorithms in a system and conducted extensive experiments that show a notable reduction in computational time relative to other graph mining methods.
\end{itemize}

We organize the paper as follows, the preliminaries are discussed in \cref{sec:preliminaries}, our approach is described in \cref{sec:approach}, our framework is described in \cref{sec:algorithm}, our results are presented in \cref{sec:results}, related works in \cref{sec:related}, and we conclude our paper in \cref{sec:conclusion}.

\section{Preliminaries}~\label{sec:preliminaries}

\subsection{General Graph Terminologies}
In this section, we give a brief explanation of the general terminologies that guide the proofs in this paper. 

\subsubsection{Articulation Vertex}

An articulation vertex (or a cut vertex) in an undirected graph is a vertex that disconnects the graph upon removal.
For a directed graph, we convert all the directed edges into undirected edges.
For example, in \cref{fig:articulation} the articulation vertex is $d_3$. Upon removal of $d_3$, the graph gets divided into three subgraphs with vertices $\set{ d_1, d_2, d_5, d_6 }$, $\set{ d_7 }$ and $\set{ d_4 }$. Mathematically, $v$ is an articulation vertex of graph $G$ iff there exist at least two other vertices $u, w$ such that there is at least one path ($\gPath{u}{w}$) from $u$ to $w$ in $G$ and  $v$ lies on every path from $u$ to $w$ in $G$.

\begin{figure}[hb]
    \centering
    \input{figures/articulation}
    \caption{Illustration of an articulation vertex}
    \label{fig:articulation}
    \ifACM
      \Description{Illustration of an articulation vertex}
    \fi
\end{figure}

\subsubsection{Subgraph isomorphism}
Let a \textbf{labeled data graph} be represented as $D(V_d, E_d, L_d)$ and a \textbf{labeled pattern graph} represented as $P(V_p, E_p, L_p)$. Then the pattern graph $P$ is subgraph isomorphic to a data graph $D$, if $|V_p| \leq |V_d|$ and if there is an injective relationship between the vertices, edges and the labels of the pattern graph and the data graph. In other words, each vertex, edge and label in the pattern graph matches to a distinct vertex, edge and label in the data graph. For instance the pattern graph in \cref{fig:example} (b) is subgraph isomorphic to the induced subgraph formed by vertices $\set{d_1, d_2, d_5}$ in \cref{fig:example} (a).

\subsection{Graph Mining}
Subgraph mining, an extension of subgraph isomorphism, is to determine all the patterns $P$ in the data graph $D$ that are \sqoutes{frequent}. A pattern graph is generated from the data graph using the relationship $V_p \subseteq V_d$, $E_p \subseteq E_d$ and $L_p \subseteq L_d$. Also, the pattern generated must be a subgraph isomorphic with the original graph. A generated pattern is frequent if it occurs over a certain threshold \acs{support} of times. In this paper, we consider single graph mining~\cite{bringmann:2008:frequent} on directed and labelled graphs. However, it is important to notice that our method can be easily extended to undirected graphs.

\begingroup
\hbadness=10000 
\begin{figure}[hb]
  \centering
  \begin{subfigure}{0.52\linewidth}
    \centering
    \resizebox{\linewidth}{!}{ 
      \input{figures/datagraph}
    }
    \caption{}
    \label{fig:datagraph}
  \end{subfigure}
  \begin{subfigure}{0.21\linewidth}
    \centering
    \resizebox{\linewidth}{!}{ 
      \input{figures/pattern/triangle1}
    }
    \caption{}
    \label{fig:patt1}
  \end{subfigure}
  \begin{subfigure}{0.21\linewidth}
    \centering
    \resizebox{\linewidth}{!}{ 
      \input{figures/pattern/triangle2}
    }
    \caption{}
    \label{fig:patt2}
  \end{subfigure}
  \caption{\subref{fig:datagraph}. Data graph $D$, \subref{fig:patt1}. Pattern graph $P_1$ \subref{fig:patt2}. Pattern graph $P_2$. Double arrow represents directed edges in both directions.}
  \label{fig:example}
  \ifACM
    \Description{Data graph $D$, Pattern graph $P_1$ and Pattern graph $P_2$}
  \fi
\end{figure}
\endgroup
\begin{figure}
  \centering
  \input{figures/diagram/mergeProcessExamplev2}
  \caption{Merge process I}
  \ifACM
    \Description{Merge process I}
  \fi
\end{figure}

\begin{figure*}
  \centering
  \runningDatagraph{0}
  \runningDatagraph{1}
  \runningDatagraph{2}
  \runningDatagraph{3}
  \runningDatagraph{4}
  \caption{Running example}
  \ifACM
    \Description{Running example}
  \fi
\end{figure*}
A general graph mining problem involves two steps. The first step is referred to as the generation step. In this step, the goal is to derive candidate subgraphs. Candidate subgraphs ${H}$ are defined as the set of all possible pattern graphs $P$ within the datagraph $D$, satisfying the condition $|V_p| \subseteq |V_d|$. For instance,~\cref{fig:patt1} and ~\cref{fig:patt2} are the subgraphs of ~\cref{fig:datagraph}. The second step is referred to as the metric step. In this step, the goal is to determine if the generated pattern graph has subgraph isomorphic patterns in the datagraph, and also to determine if the frequency of the occurrence of the pattern graph, is over a certain threshold (referred to as support 
value) \acs{support}. For instance, in the ~\cref{fig:example}, the subgraphs $\set{d_1, d_2, d_5}$, $\set{d_2, d_3, d_6}$ and $\set{d_3, d_4, d_7}$ are all subgraph isomorphic to $\set{u_1, u_3, u_2}$. However, if we consider a threshold of $4$, then Pattern $P_1$ is not frequent in $D$.

\subsubsection{Anti-monotone Property}
Let there be two subgraphs $P$ and $Q$ of data graph $D$ such that $P \subset Q$ and $V_p \cup x = Q$ where $x$ is a vertex in $D$. Anti-monotone property states the $\FunctionCall{Freq}{P} \geq \FunctionCall{Freq}{Q}$.

\subsection{Merging algorithm terminologies}
In the generation step, all possible candidates are generated. There have been many pruning methods that have been explored in the literature~\cite{elseidy:2014:grami}. In this section we give the basic terminologies required for the novel pruning method that we introduce in this paper.

\begin{figure}[htb]
  \centering
  \begin{subfigure}{0.28\linewidth}
    \centering
    \input{figures/core/core1u1}
    \caption{CoreGraph $C_1^{u1}$}
    \label{fig:core:c1u1}
  \end{subfigure}
  \begin{subfigure}{0.28\linewidth}
    \centering
    \input{figures/core/core1u2}
    \caption{CoreGraph $C_1^{u2}$}
    \label{fig:core:c1u2}
  \end{subfigure}
  \begin{subfigure}{0.33\linewidth}
    \centering
    \input{figures/extendedCore/e1u1}
    \caption{ext CoreGraph $E_1^{u1}$}
    \label{fig:ext:core:e1}
  \end{subfigure}
  \caption{CoreGraphs \& extended CoreGraph for pattern $P_1$}
  \label{fig:core:example}
  \ifACM
    \Description{CoreGraphs \& extended CoreGraph for pattern $P_1$}
  \fi
\end{figure}

\subsubsection{CoreGraph}
We define CoreGraph as a pattern graph with one disconnected vertex. For instance in \cref{fig:core:c1u1}, the vertices $\set{u_3, u_2}$ are connected and the vertex $\set{u_1}$ is disconnected, the CoreGraph in this setting is all the three vertices together. The CoreGraph (\cref{fig:core:c1u1}) is formed by  disconnecting vertex $\set{u_1}$ from pattern $P_1$ is denoted by $C_1^{u1}$. We use $C_m^{u_j}$ to denote a CoreGraph formed by disconnecting $u_j$ vertex from the pattern graph $P_m$.

\subsubsection{Marked Vertex}
The vertex $\set{u_1}$ that was disconnected from the pattern $P_1$ to form the CoreGraph is referred to as the marked vertex of the CoreGraph.

\subsubsection{Isomorphism in CoreGraph}
In order for two CoreGraphs to be isomorphic, the subgraph formed by removing the one vertex must be isomorphic. That is, for two core $C_m^{uj}$ and $C_n^{uk}$ are isomorphic iff the graphs formed by removing the vertex $u_j$ from $P_m$ and vertex $u_k$ from $P_n$ are isomorphic. For example, $C_1^{u1}$ is isomorphic to $C_1^{u3}$.

\subsubsection{AllCores}
AllCores is an array that contains all the CoreGraphs formed from all the patterns of the same size. That is, if we assume that $P_1$ and $P_2$ are the only size $3$ patterns, $AllCores$ will be $\set{C_1^{u1}, C_1^{u2}, C_1^{u3}, C_2^{u1}, C_2^{u2}, C_2^{u4}}$.

\subsubsection{CoreMap}
A CoreMap in a pattern graph refers to a collection of CoreGraphs that are generated from the given pattern. For instance, $CoreMap(P_1)$ will be $\set{C_1^{u1}, C_1^{u2}}$. Since $C_1^{u3}$ is isomorphic to $C_1^{u1}$ it is not included in the CoreMap.

\subsubsection{CoreGroup}

A CoreGroup is collection of all the CoreGraphs that are generated from patterns of same size. They group the CoreGraphs which are isomorphic within same group. CoreGroup created from pattern graph $P_1$ and $P_2$ (\cref{fig:patt1} and \cref{fig:patt2}) would contain $CoreGroup(C_1^{u3}) = \set{C_1^{u3}, C_1^{u1}}, CoreGroup(C_1^{u2}) = \set{C_1^{u2}}$ and so on.

\subsection{Metric Step}
The metric step is the second phase of graph mining. During this step, the goal is to identify which among the candidate patterns that were generated are actually considered frequent. In the literature, two metrics are defined for graph mining, Maximum Independent Set (MIS)~\cite{kuramochi:2005:finding} and Minimum Image based (\ac{mni})~\cite{bringmann:2008:frequent}. A variation of the \ac{mni} method, known as Fractional Score~\cite{yuan:2023:tfsm} has also been proposed. In this section we define these metrics along with our metric.

\subsubsection{Independent Set}
A set represents a collection of all the vertex mappings from the data graph to the pattern graph. For example, in \cref{fig:example}, if we consider pattern $P_1$, the set of mappings would be $\set{d_1, d_2, d_5}$, $\set{d_2, d_3, d_6}$ or $\set{d_3, d_4, d_7}$. Now, an independent set is a subset of this mapping set that only includes mappings without any overlapping vertices. In the case of pattern $P_1$, an independent set could be $\is{\set{d_1, d_2, d_5}, \set{d_3, d_4, d_7}}$, $\is{\set{d_2, d_3, d_6}}$, $\is{\set{d_1, d_2, d_5}}$, or $\is{\set{d_3, d_4, d_7}}$.

\subsubsection{\acf{mal}}
 \ac{mal} is a subset of all the independent sets, where no additional mappings can be added without violating the independence property. For instance, in \cref{fig:example}, for pattern $P_1$, $\is{\set{d_2, d_3, d_6}}$ is a maximal independent set, however, $\is{\set{d_1, d_2, d_5}}$ is not, since $\set{d_3, d_4, d_7}$ can be added without violating the property of independent sets. 
 
\subsubsection{\acf{mis}}
A \acf{mis}~\cite{kuramochi:2005:finding} is the independent set with the largest number of mappings. For instance, in \cref{fig:example}, $\is{\set{d_1, d_2, d_5}, \set{d_3, d_4, d_7}}$ is a MIS but $\is{\set{d_2, d_3, d_6}}$ is not.

\subsubsection{\acf{mni}}
A \ac{mni} method~\cite{bringmann:2008:frequent} is a set of all possible mappings from the datagraph to the pattern graph. That is the independence is not considered. For instance, the \ac{mni} metric, for \cref{fig:example} is $\is{\set{d_1, d_2, d_5}$, $\set{d_2, d_3, d_6}$, $\set{d_3, d_4, d_7}}$. Thus, when compared to the previous two metrics, \ac{mni} overestimates the support value.

\subsubsection{Fractional-Score}
A Fractional Score~\cite{yuan:2023:tfsm} based method is an extension of \ac{mni}, which uses fractional score to reduce overestimation. The fractional score is determined based on the contribution of each vertex to its neighbors. For instance, in ~\cref{fig:example}, for datagraph $D$ and pattern graph $P_1$ the contribution of $d_5$ to $d_1$ is $1/2$, this is because there are two vertices with the same label that $d_5$ can equally contribute to. With this value the total contribution of each vertex to a specific label is calculated, in our case, the total fractional contribution to $d_1$ from all neighbors with label \sqoutes{Blue} is $1/2$. Finally, this value is used to deduce the fractional contribution of all vertices of pattern graph $P_1$ as $3$. It is imperative to notice that this value should have actually been $2$ according to MIS. Thus, even though for specified examples this method is closer to the MIS value, it is not always the case as shown in our example.

\subsubsection{Comparison between the metrics}
The Maximum Independent Set (MIS) is considered the gold standard because it provides the exact count of repetitions for a specific pattern. However, solving MIS problem is challenging. The \ac{mni} metric is an approximation of MIS and offers a quicker solution. However, \ac{mni} has a tendency to overestimate the presence of certain patterns in the graph while sometimes failing to count automorphic patterns accurately. An extension called the Fractional-Score metric attempts to balance these issues, however it still overestimates the presence of some patterns.

As a more suitable metric for Subgraph Mining, we propose to use \ac{mal}. It preserves the crucial independent set property of MIS and provides the flexibility to choose between overestimation or underestimation of patterns (using a slider value). Additionally, \ac{mal} has the advantage of running with similar runtimes as \ac{mni}, making it a practical choice for subgraph mining tasks.

\section{FLEXIS}~\label{sec:flexis}

The \ac{flexis} framework presents an innovative approach for discovering frequent subgraphs within a data graph. This framework is built upon the concept of merging two prevalent $(k-1)$-vertex patterns to potentially identify a $k$-vertex pattern. It introduces a user-defined parameter referred to as the \textit{slider value} to finely regulate the degree of overlap between patterns identified by the \ac{mis} and \ac{mal}. Additionally, it incorporates a novel pruning technique aimed at curtailing the search space by reducing the number of candidate patterns under consideration.

\subsection{Methodological Contributions}

As in~\cite{kuramochi:2005:finding} we combine two $k-1$ frequent patterns to find possible $k$ frequent patterns. However, in~\cite{kuramochi:2005:finding} the size of the pattern graph is defined based on the number of edges in the graph, whereas in ours the size is defined based on vertices. For instance, a pattern graph with 3 vertices and 2 edges will be considered in size 2 in their method and size 3 in our method. This classification is important as it helps in effective pruning of the search space, which in turn helps in better performance of our method.

Apart from this we also introduce a new metric \ac{mal} which selectively adapts the best of the other two metrics \ac{mis} and \ac{mni}. It adapts the non-overlapping vertices property from \ac{mis}, which is not true in the case of \ac{mni}, thus making sure that there is no over-estimation of the number of patterns in the data graph, a most commonly known issue in the predominantly used \ac{mni} metric~\cite{yuan:2023:tfsm}. Also, it adapts the property of finishing the search in a reasonable amount of time for graphs with a large number of vertices from \ac{mni}, which is not true in the case of \ac{mis}, attributed to the NP-hardness of the problem. Apart from this we also provide a slider value, a user-controlled parameter, which allows the user to tune the accuracy-speed trade-off of the algorithm.

Thus, we define frequent subgraph matching as follows, given a data graph $D$, support value $\sigma$, and a slider value $\lambda$, find all the subgraphs in $D$ that occur at least $\tau$ times, where $\tau$ is dependent on $\sigma$ and $\lambda$. It is imperative to note here that our definition is different from the general definition of frequent subgraph mining, which determines all the frequent patterns in $D$ that occur at least $\sigma$ times. To the best of our knowledge, this is the first time that a user-controlled parameter has been introduced in the context of frequent subgraph mining. We next formally define the \ac{mal} metric and the slider value and provide an example to illustrate our method. 

\begin{mydef}
  \label{def:mal}
 \acf{mal} is a subset of all the independent sets, where no additional mappings can be added without violating the independence property. For instance, in \cref{fig:datagraph}, for pattern $P_1$, $\is{\set{d_2, d_3, d_6}}$ is a maximal independent set, however, $\is{\set{d_1, d_2, d_5}}$ is not, since $\set{d_3, d_4, d_7}$ can be added without violating the property of independent sets. 

\end{mydef}

\begin{mydef}
  \label{def:slider}
  To incorporate \ac{mal} instead of \ac{mis} we use a slider ($\lambda$), which is defined by the user and is in the range of $[0.0, 1.0]$. With this user-defined slider, we determine $\tau$ as the linear interpolation dependent on the provided $\lambda$, the number of vertices in the candidate pattern $n$ and the required support value $\sigma$. Precisely, $\tau = \sigma (1 - 1/n) \lambda + \sigma/n$. 
\end{mydef}

  For instance, if the user provides $lambda = 0.4$ and the support value $\sigma = 600$ and the considered candidate pattern has $3$ vertices, then $\tau = 360$. Thus, \ac{flexis} will have to find at least $360$ matches for the candidate pattern to be considered frequent, as opposed to $600$ matches in the case of \ac{mis}. This provides the necessary approximation for speedup, while also ensuring that no frequent patterns are missed.

\ac{flexis} starts with finding the matches for all the edges in the data graph. After getting all the two edge pattern graphs, it sees which of them are frequent by using a matcher (vf3matcher). After finding the frequent patterns, it merges all the frequent patterns of size $2$ into candidate patterns of size $3$. \ac{flexis} repeats the steps of 
\begin{enumerate*}[label=\roman*)]
  \item finding the frequent patterns, and
  \item merging frequent patterns till maximum size is reached or no candidate patterns remain.
\end{enumerate*}

To understand each of the contributions in detail, let us consider \cref{fig:datagraph} as data graph, and \cref{fig:patt1} as the current candidate pattern under consideration. Let us assume that the support value $\lambda = 1.0$. Consider the following two cases:
\begin{enumerate}
  \item For the support value $\sigma = 3$, according to the definition of \ac{mis} and \ac{mal}, matchings for the candidate pattern graph in the data graph will be as shown in \cref{fig:dataGraphMappingMIS} and \cref{fig:dataGraphMapping4} respectively. Thus for the defined parameters both the \ac{mis} and \ac{mal} will estimate that the candidate pattern is not frequent. Whereas \ac{mni} will match as shown in \cref{fig:dataGraphMappingMNI}. Hence, it will conclude the pattern to be frequent. This is because of \ac{mni} considering overlapping vertices.
  
  \item In the case of the methods that use \ac{mni} as the metric the number of candidate search spaces will increase faster when compared to our method. That is the number of candidate patterns that are searched in the case of \ac{mni} is more when compared to our method, as shown in \cref{tab:searchedPatterns}. This gives our method the pruning ability, which in turn helps in speeding up the search process.
\end{enumerate}
Now let us consider, how the value of $\lambda$ affects the search process. In the case where $\sigma = 2$ and $\lambda = 1$, $\tau$ will be $2$, \ac{flexis} can find either \cref{fig:dataGraphMapping3} or \cref{fig:dataGraphMapping4}. In the case of \cref{fig:dataGraphMapping3}, the pattern graph will be declared non-frequent, whereas in the case of \cref{fig:dataGraphMapping4} the pattern graph will be declared frequent. Thus, in this case, we either underestimate or correctly estimate if a pattern is frequent or not. In another case, where $\sigma = 2$ and $\lambda = 0.25$, $\tau$ for 3-size pattern will be $1$. In this case, \ac{flexis} will find \cref{fig:dataGraphMapping1}, \cref{fig:dataGraphMapping2}, and \cref{fig:dataGraphMapping3}. Thus, in this case, \ac{flexis} correctly estimates that the pattern is frequent. Similarly, for some values of $\lambda$, our method can overestimate the number of frequent patterns. This is similar to approximation to $\ac{mni}$, where the metric overestimates or correctly estimates the number of frequent patterns. But never finds a wrong frequent pattern. It is this property that gives \ac{flexis} the ability to run faster than \ac{mis}.

To understand our second contribution, let us consider pattern graphs $\cref{fig:patt1}$ and $\cref{fig:patt2}$ to be frequent, then \ac{flexis} will merge these patterns (explained in \cref{sec:algorithm}) to form a new candidate pattern graph as shown in \cref{fig:mergeProcessExamplev2}. This method is different from the existing method~\cite{kuramochi:2005:finding}, as they combine two $k-1$ frequent patterns based on the number of edges instead of vertices. The advantage of \ac{flexis} is the pruning of search space is more efficient. For instance, in a data graph with $40$ vertices, the support $\sigma = 10$, the candidate pattern graph can have at most $4$ vertices with no vertex overlap. \ac{flexis} can thus prune, all the candidate patterns after $3^{rd}$ merging step, whereas their case~\cite{kuramochi:2005:finding} the pruning will require more merging steps. Thus, our method speeds up the search process. We differ from GraMi~\cite{elseidy:2014:grami} and T-FSM~\cite{yuan:2023:tfsm}, as they do not use merging to two frequent patterns to find the next candidate pattern. They extend the frequent patterns by adding a new edge to generate the next candidate patterns. Since combining two frequent graphs generates a lesser number of candidate patterns, our method is more efficient than GraMi and T-FSM.

Thus, our method has the following advantages,
\begin{enumerate*}
  \item \ac{mal} is more closely related to the actual frequent pattern count metric \ac{mis}; while providing the same or better speedup than \ac{mni}.
  \item \ac{mal} is the first metric that allows the user to control the accuracy-speed trade-off.
  \item \ac{flexis} is the first method that uses the merging of two frequent patterns to find the next candidate pattern, based on the number of edges instead of vertices. And thus, providing a more efficient pruning of the search space. Hence, speeding up the search process.
\end{enumerate*}

\begin{figure}[htb]
  \centering
  \input{figures/diagram/mergeProcessExamplev2}
  \caption{Merge process I}
  \label{fig:mergeProcessExamplev2}
  \ifACM
    \Description{Merge process I}
  \fi
\end{figure}

\begin{figure}[htb]
  \centering
  \begin{subfigure}{0.495\textwidth}
    \centering
    \runningDatagraph{5}
    \caption{Mapping I}
    \label{fig:dataGraphMapping1}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
    \centering
    \runningDatagraph{6}
    \caption{Mapping II}
    \label{fig:dataGraphMapping2}
  \end{subfigure}
  \caption{\ac{flexis} mappings I}
  \ifACM
    \Description{Maximal Independent Set mappings}
  \fi
\end{figure}
\begin{figure}[htb]
  \begin{subfigure}{0.495\textwidth}
    \centering
    \runningDatagraph{2}
    \caption{Mapping III}
    \label{fig:dataGraphMapping3}
  \end{subfigure}
  \begin{subfigure}{0.495\textwidth}
    \centering
    \runningDatagraph{1}
    \caption{Mapping IV}
    \label{fig:dataGraphMapping4}
  \end{subfigure}
  \caption{\ac{flexis} mappings II}
  \ifACM
    \Description{Maximal Independent Set mappings}
  \fi
\end{figure}

\begin{figure}[hb]
  \centering
  \begin{subfigure}{0.495\linewidth}
    \centering
    \runningDatagraph{7}
    \caption{\ac{mni} mapping}
    \label{fig:dataGraphMappingMNI}
  \end{subfigure}
  \begin{subfigure}{0.495\linewidth}
    \centering
    \runningDatagraph{1}
    \caption{\ac{mis} mapping}
    \label{fig:dataGraphMappingMIS}
  \end{subfigure}
  \caption{\ac{mni} and \ac{mis} mappings}
  \ifACM
    \Description{MNI and MIS mappings}
  \fi
\end{figure}

\begin{table}
  \input{tabular/searchedPatterns-0.5}
  \caption{Searched patterns}
  \label{tab:searchedPatterns}
  Number of searched patterns for different support values for Gnutella.
  $|S_g|$ for MNI,
  $|S_f|$ for \acs{mal}, and 
  $|S_t|$ for MNI-Fractional.
  T-FSM's version of MNI is used due its higher efficiency than GraMi~\cite{yuan:2023:tfsm}.
\end{table}

\begin{figure*}[htb]
  \centering
  \runningDatagraph{0}
  \runningDatagraph{1}
  \runningDatagraph{2}
  % \runningDatagraph{3}
  % \runningDatagraph{4}
  \caption{Running example}
  \ifACM
    \Description{Running example}
  \fi
\end{figure*}

\subsection{Algorithmic flow of FLEXIS}~\label{sec:algorithm}

The flow of \ac{flexis} is illustrated in \cref{alg:mining}. The main algorithm has two main parts,
\begin{enumerate*}[label=\roman*)]
  \item \textbf{Generation Step}: This phase generates candidate patterns either directly from the data graph $G$ or based on frequent patterns obtained in the previous step ($FP$).
  \item \textbf{Metric Step}: Subsequently, candidate patterns are assessed for their frequency within the data graph $G$
  \end{enumerate*}

  The \ac{flexis} framework, outlined in \cref{alg:mining}, operates in the following manner:
  
  \begin{enumerate}
      \item Candidate Pattern Generation (Generation Step): Initially, \ac{flexis} generates all size-2 candidate patterns ($CP$) from the data graph $G$, which essentially includes all edges within the data graph (see \cref{alg:mining:edges}).
      \item Finding Frequent Patterns (Metric Step): To identify frequent patterns ($FP$) within the candidate set, \ac{flexis} utilizes a modified version of Vf3Light~\cite{carletti:2018:vf3,carletti:2019:vf3}, integrating our custom metric \ac{mal}. This metric ensures non-overlapping matches and enables user control over the trade-off between accuracy and speed (refer to \cref{sec:matcher_step})
      \item Candidate Pattern Expansion (Next Generation Step): Subsequently, \ac{flexis} combines the detected frequent patterns ($FP$) to generate the next level of candidate patterns ($CP$) (\textbf{Generation Step}). This iterative process continues until it reaches either the maximum pattern size (as outlined in \cref{alg:mining:stop}) or exhausts all unexplored patterns (\cref{alg:mining:loop})
  \end{enumerate}
  
  Our approach deviates from the traditional implementation of Vf3Light~\cite{carletti:2018:vf3,carletti:2019:vf3}, which employs the \ac{mni} metric, allowing automorphism and overlapping vertices. In contrast, our adaptation of Vf3Light integrates our metric \ac{mal} to ensure non-overlapping vertices.
  





% \ac{flexis} first generates all the candidate patterns $CP$ of size $2$ from the data graph $G$ (\cref{alg:mining:edges}) which are all the edges in the data graph (\textbf{Generation step}). Then it uses a matcher to find the frequent patterns $FP$ from these candidate patterns (\cref{alg:mining:matcher}). To find the frequent patterns, \ac{flexis} uses modified version of Vf3Light~\cite{carletti:2018:vf3,carletti:2019:vf3} (\cref{alg:mining:merger}) to determine the frequent patterns (\textbf{Metric step}). After finding the frequent patterns, \ac{flexis} merges the frequent patterns $FP$ to form the next level of candidate patterns $CP$ (\textbf{Generation Step}). This process continues until either the patterns of maximum size (\cref{alg:mining:stop}) are searched or there are no more patterns left to explore (\cref{alg:mining:loop}).

% Whether a pattern is frequent or not is determined by our defined metric \ac{mal}, which avoids overlapping vertices in the matches and allows a user-defined parameter $\lambda$ to control the accuracy-speed trade-off, we further explain this in the \cref{sec:matcher_step}. Since, our method required non-overlapping vertices, which is different from the existing implementation of Vf3Light~\cite{carletti:2018:vf3,carletti:2019:vf3}, which uses \ac{mni} metric, and hence contains automorphism and overlapping vertices, we modified the Vf3Light to use our metric \ac{mal}.


% The flow of our overall algorithm, referred to as \ac{flexis}, is illustrated in \cref{alg:mining}. In the initial step (\cref{alg:mining:edges}), the algorithm selects all the edges in the data graph as candidate pattern graphs, using the \FunctionCall{edges}{G}.
% Subsequently, we use \Call{vf3Matcher}{} a modified version of Vf3Light~\cite{carletti:2018:vf3, carletti:2019:vf3} to determine the matches.
% \changed{Vf3Light uses \ac{mni} metric instead of \ac{mis} metric. As a result, the matches contain automorphisms and vertices might be shared across different matches which is counterproductive in the context of the \ac{mal} metric.}

% To address these issues, our \ac{mal} metric is applied to candidate patterns ($CP$) 
% All these anomalies are dealt with in the candidate patterns ($CP$) using our \ac{mal} metric, taking into account both the support \acs{support} and \ac{lerp}. The set of these frequent subgraphs is denoted by $FP$. The patterns identified as frequent ($FP$) are then combined using our novel method to generate the next level of candidate patterns (\cref{alg:mining:merger}). This process continues until either the patterns of maximum size (maxStep) are searched or there are no more patterns left to explore.
\begin{algorithm}
  \caption{\ac{flexis}}
  \label{alg:mining}
  \input{algorithms/mining}
\end{algorithm}

We explain in detail our approach in the Generation and the Metric Steps, in the following sections. 

\subsubsection{Generation Step}

In \ac{flexis}, the candidate patterns are generated by combining, frequent size $(k-1)$-vertex patterns to form size $k$-vertex pattern. We premise our approach on the fact that smaller graphs can be combined to form a larger graph and for the larger graph to be frequent the smaller graphs must have been frequent (i.e., \ac{mal} is anti-monotone). For $k$ to be frequent, any subgraph of size $(k-1)$ must also be frequent.

We explain in detail how these pattern candidates are formed and prove that it is feasible to form these candidates for all the graphs in this section.

\begin{lemma}~\label{lemma:dia}
  Let $G$ be a connected graph with more than $2$ vertices. Let $u$ and $v$ be $2$ vertices of $G$ whose distance from each other is equal to diameter of $G$ ($d(u, v) = dia(G)$). Then according to the proof~\cite{kingan:2022:GraphsAndNetworks,Clark:2005:AFirstLookAtGraphTheory} $u$ and $v$ are \ac{nav} of $G$.
\end{lemma}

\begin{lemma}~\label{lemma:nAV}
  In a non-clique graph, with at least three vertices there are at least two \ac{nav} that are not connected to each other.
\end{lemma}
\begin{lemma}~\label{lemma:candidateGeneration}
  Every non-clique $k$-size candidate pattern graph can be generated by using $(k-1)$-size frequent patterns.
\end{lemma}
\begin{theorem}~\label{theo:candidateGeneration}
  Every non-clique candidate pattern can be generated by using our method.
\end{theorem}

\paragraph{Forming a CoreGraph} 
The first step for merging, frequent $(k-1)$ size patterns to form $k$ size pattern, is forming the CoreGraph. For this, we generate all possible CoreGraphs (\cref{theo:candidateGeneration}) of all frequently occurring $(k-1)$ patterns. Each of these patterns will generate $k-1$ CoreGraphs with each vertex being removed once. Out of all the CoreGraphs that are generated only the unique ones are recorded. 

To determine if a particular CoreGraph ($C_{k-1}^{x}$) is unique, we use Bliss~\cite{JunttilaKaski:ALENEX:2007:bliss, JunttilaKaski:TAPAS:2011:bliss}. Bliss generates a canonical representation of the pattern graph.  Unfortunately, Bliss cannot handle edge labels and bi-directed edges, mandating the need to determine extended CoreGraphs ($E_{k-1}^{x}$). In an extended CoreGraph, the edges are also converted into vertices and the vertex label is kept the same as the edge label. That is, for each edge $(u, v) \in C_{k-1}^{x}$, we generate new vertex $w$ such that $\FunctionCall{L}{w}$ is $\FunctionCall{L}{u, v}$, and insert edges $(u, w)$ and $(w, v)$ in the $E_{k-1}^{x}$. For instance, the extended CoreGraph \cref{fig:ext:core:e1} is an extension of CoreGraph \cref{fig:core:c1u1}, in which the edge from $u_3$ to $u_2$ is converted into $u_4$ and the edge from $u_2$ to $u_3$ is converted to $u_5$.

Upon giving the extended CoreGraph to Bliss, a canonical form of the graph and a hash for the graph is created. The hash that is generated by Bliss is used to determine the uniqueness of the CoreGraph. Note, CoreGraphs $C_1^{u_1}$ and $C_1^{u_3}$ would be the same, so the set will contain only one of them. However, even though the CoreGraphs $C_2^{u_2}$ and $C_2^{u_4}$ are the same, since they generate from different patterns, a copy of each will be maintained. 

The generated CoreGraphs are combined to form a bigger candidate pattern graph, as described below.
For the rest of the paper, we will assume CoreGraph $C_{k-1}^{x}$ to be extended CoreGraph $E_{k-1}^{x}$.

\paragraph{Merging two k-1 pattern graphs to form a k-size pattern graph}

\begin{figure}[htb]
  \centering
  \input{figures/diagram/mergeProcessExample}
  \caption{Visualization of merging process}
  \label{fig:core:mergeProcess}
  \ifACM
    \Description{Visualization of merging process}
  \fi
\end{figure}

The overview of merging two $(k-1)$-size patterns to form a k-size pattern graph is as shown in \cref{fig:core:mergeProcess}.
The above-mentioned procedure is used for the formation of core graphs, which, as shown in \cref{fig:core:mergeProcess}, consist of a $(k-2)$ sized graph and a separately marked vertex (indicated by a dotted circle).
To generate non-clique candidate patterns, we combine two core graphs that share an isomorphic $k-2$ sized graph.
To establish a clique pattern, we ascertain the existence of a third core graph in which the marked vertices of the other two cores are interconnected.

Before we explain the exact algorithms used to accomplish this merging procedure, we first establish that it's always possible to split a non-clique $k$-vertex graph into two $k-1$ vertex graphs by isolating the graph at its two non-Articulation Vertex (\ac{nav}), that are not connected. We reason that if we can split a graph into two smaller parts, we can apply the reverse principle to merge two $k-1$ size graphs into a larger $k$ size graph. We propose a different method for cliques.

Thus, based on the previous \cref{lemma:nAV}, we can split the $k$ size graph into two $(k-1)$ size graphs at the unconnected \ac{nav}.
So from the anti-monotone property, we can state that for the $k$ graph to be frequent the two $(k-1)$ graphs formed by splitting must have also been frequent.
Thus, we can put together the two $(k-1)$ graphs in all possible ways to get all the possible candidates for $k$-size patterns.
The main idea of generating $k$-size patterns is shown in \cref{fig:core:mergeProcess}.

\paragraph{Merging non-cliques}

\paragraph{Merging cliques}
\begin{figure}[htb]
  \centering
  \begin{subfigure}{0.30\linewidth}
    \centering
    \input{figures/pattern/merged11}
    \caption{$C_1^{u_1} \cup C_1^{u_1}$}
  \end{subfigure}
  \begin{subfigure}{0.30\linewidth}
    \centering
    \input{figures/pattern/merged11_2}
    \caption{$C_1^{u_2} \cup C_1^{u_2}$}
    \label{merged:pattern:c1u2c1u2}
  \end{subfigure}
  \begin{subfigure}{0.30\linewidth}
    \centering
    \input{figures/pattern/merged12}
    \caption{$C_1^{u_1} \cup C_2^{u_2}$}
    \label{fig:mergePatt3}
  \end{subfigure}
  
  \caption{$\cup$ refers to merging to corresponding CoreGraphs}
  \label{fig:merge:patternResultant}
  \ifACM
    \Description{$\cup$ refers to merging to corresponding CoreGraphs}
  \fi
\end{figure}

To comprehensively elucidate our approach, let us commence by establishing the correlation between CoreGraphs and the associated proofs.
To facilitate this, we consider a graph of size $k$, as shown in \cref{fig:mergePatt3}.
As per the \cref{lemma:nAV}, there must exist two \ac{nav} within this graph that are disconnected. In the example, these vertices are $u_3$ and $u_4$. We reduce the 4-sized pattern graphs into two 3-sized pattern graphs by removing the \ac{nav}. Consequently, removing the \ac{nav} yields $P_1$ and $P_2$ as shown in \cref{fig:patt1} and \cref{fig:patt2} respectively. An essential observation to make within these patterns lies in the outcome of removing vertices $u_3$ and $u_4$ alongside their associated edges. This action results in isomorphic smaller graphs, each possessing a size of $k-2$. This $k-2$ pattern, in conjunction with the isolated vertex, is denoted as the CoreGraph. Therefore, when we undertake the reverse process of merging two $k-1$ sized graphs to formulate a $k$ sized graph, it suffices to identify the isomorphic CoreGraphs. Subsequently, we can execute the graph merger by incorporating the isolated vertices extracted from both constituent graphs. This precise methodology constitutes how we merge two $k-1$ size graphs to construct a $k$ size graph.

As mentioned in the proof, clique is a special condition.
To determine if Clique is a possible candidate pattern, we need to determine if there exists another CoreGraph in the list that allows us to connect the disconnected \ac{nav}.
Thus, for Cliques, three patterns are required.
For instance, using our method for non-cliques, from patterns $P_1$ and $P_2$ (\cref{fig:example}), we can generate all the figures from \cref{fig:merge:patternResultant}.
But, as it can be seen we are missing $\gPath{u_1}{u_4}$, $\gPath{u_2}{u_4}$, and $\gPath{u_3}{u_4}$.
However, considering the CoreGraphs  $C_1^{u2}, C_2^{u1},$ and $C_1^{u1}$, we can generate the clique.

Thus, the generation of a clique differs from a non-clique by only one CoreGraph.

\begin{figure}[htb]
    \centering
  \begin{subfigure}{0.30\linewidth}
    \centering
    \input{figures/pattern/tailTri1}
    \caption{Pattern graph $P_t$}
    \label{fig:tailTri}
  \end{subfigure}
  \begin{subfigure}{0.30\linewidth}
    \centering
    \input{figures/pattern/mergeTailTri1}
    \caption{Merged graph $P_{t1}$}
    \label{fig:mergeTri1}
  \end{subfigure}
  \begin{subfigure}{0.30\linewidth}
    \centering
    \input{figures/pattern/mergeTailTri2}
    \caption{Merged graph $P_{t2}$}
    \label{fig:mergeTri2}
  \end{subfigure}
    \caption{All permutations}
    \label{fig:trailedTriangle}
    \ifACM
      \Description{All permutations}
    \fi
\end{figure}

\paragraph{Proposed Algorithms}

\begin{algorithm}
  \caption{Candidate Pattern Generation}
  \label{alg:generate:New:Patterns:nonclique}
  \input{algorithms/generateNewPatterns}
\end{algorithm}

To generate the candidate pattern for size $k$ from size $k-1$ graphs using CoreGraphs generated by $k$ size patterns, we follow \cref{alg:generate:New:Patterns:nonclique}. First, the CoreGraphs are put together to form a CoreGroup (defined above) as in \cref{alg:gen:nc:cg:gen}. Then, we iterate through all the graphs in the CoreGroup. For each graph, we check, if the marked vertex can be connected in various ways to one of the CoreGraphs. If the vertex can be connected only in one configuration then autos contain that configuration otherwise it will contain all the configurations possible (\cref{alg:gen:nc:fa}). These configurations are iterated by the algorithm and used to generate different pattern graphs at \cref{alg:gen:nc:ma}. Lastly, \cref{alg:gen:nc:gnc} generates new cliques. We explain the three core components of this algorithm, namely, \FunctionCall{findAutomorphism}{}, \FunctionCall{merge}{} and \FunctionCall{generateNewClique}{} in the following sections.

\cref{alg:core:findautomorphism}, \FunctionCall{findAutomorphism}{} uses generators produced by Bliss~\cite{JunttilaKaski:TAPAS:2011:bliss, JunttilaKaski:ALENEX:2007:bliss} in \cref{alg:fa:gen}. Generators can be used to generate automorphisms of the CoreGraph. The algorithm iterates through all the CoreGraphs and generators while checking if different connections with marked vertex are possible (\cref{alg:fa:dt}). If different connections are possible then the algorithm returns all the automorphisms, otherwise, it returns the identity permutation.
For instance, generator for $C_1^{u_2}$ are shown in \cref{tab:generator:c1}.
\changed{Generators can be used to generate different permutations of the CoreGraph. Different permutations are shown in \cref{tab:permutation:c1}.}.

\begin{table}[hb]
  \caption{generator and permutations of the graph}
  \begin{subtable}[b]{0.45\linewidth}
    \centering
    \caption{generator for $C_1^{u_2}$}
    \label{tab:generator:c1}
    \input{tabular/generator}
  \end{subtable}
  \begin{subtable}[b]{0.45\linewidth}
    \centering
    \caption{permutations of $C_1^{u_2}$}
    \label{tab:permutation:c1}
    \input{tabular/permutation}
  \end{subtable}
 \end{table}

\begin{algorithm}[H]
  \caption{checks if merged in different configs possible}
  \label{alg:core:findautomorphism}
  \input{algorithms/findAutomorphism}
\end{algorithm}

\cref{alg:core:diffTopo} is used to check if marked vertex can be connected via different topologies.

Let's consider a CoreGraph $C_n^{u_m}$. The algorithm first converts the CoreGraph into graph in Bliss's canonical mapping via \cref{tab:canon:c1}. Then, the algorithm transforms the vertices (neighbors of marked vertex) via generators. It then converts from Bliss's canonical form back to CoreGraph via \textbf{I} (\cref{tab:inverse:c1}). After transformations, the algorithm checks if marked vertex is being connected to same neighboring vertices or not (\cref{alg:line:dt:return}).

\begin{table}[b]
  \centering
  \caption{Canonical and Inv. canonical form from $C_1^{u_2}$ \& to $C_1^{u_2}$}
  \label{tab:canoninverse:c1}
  \begin{subtable}[b]{0.43\linewidth}
    \caption{Canonical form \textbf{C}}
    \label{tab:canon:c1}
    \input{tabular/canon}
  \end{subtable}
  \begin{subtable}[b]{0.55\linewidth}
    \caption{Inv. canonical form \textbf{I}}
    \label{tab:inverse:c1}
    \input{tabular/inverse}
  \end{subtable}
\end{table}

\begin{algorithm}[ht]
  \caption{Generating different permutation of same graph $C_n^{u_m}$}
  \label{alg:core:diffTopo}
  \input{algorithms/differentTopology}
\end{algorithm}

After generating the different permutations using \cref{alg:core:findautomorphism} and \cref{alg:core:diffTopo}, we merge the two graphs to form a new pattern graph. The algorithm for merging is shown in \cref{alg:mergecore:nonclique}.
The algorithm first obtains the original pattern from one of the CoreGraphs by attaching its marked vertex (\cref{algo:line:cg:marked}).
It then generates a new vertex that has the same label as the marked vertex of other CoreGraph (\cref{algo:line:other:marked}).
The algorithm uses $gen$ to generate different edge configurations of the marked vertex (\cref{algo:merge:line:perm}). It then converts the neighbors back to CoreGraph space via (\cref{algo:merge:line:inverse}).

After transforming the vertices, it inserts corresponding edges to the new pattern graph ($np$) at \cref{algo:line:other:addedge}. Lastly, it returns the new pattern graph $np$.

\begin{algorithm}
  \caption{merging CoreGraphs to generate new patterns}
  \label{alg:mergecore:nonclique}
  \input{algorithms/merge}
\end{algorithm}

Since the method to generate new patterns is different for cliques, we propose \cref{alg:generateNewCliques} \FunctionCall{generateNewCliques}{} generates cliques given the intermediate data from \cref{alg:generate:New:Patterns:nonclique}. First, the algorithm makes sure that the identified CoreGraphs $i$ and $j$ are from clique patterns (\cref{alg:line:cl:cliques}). $mv$ is another vertex from CoreGraph $i$ which is not marked vertex (\cref{alg:line:cl:otherV}). Next $cliqBase$ is the CoreGraph with $mv$ as a marked vertex (\cref{alg:line:cl:cliqBase}). $auto2s$ will contain all the permutations of automorphism in \cref{alg:line:cl:fa}. Then, the algorithm calls \FunctionCall{mergeClique}{} (\cref{alg:line:cl:merge}) to merge and generate the clique. Lastly, if the valid clique is found, then its added the $P_{k+1}$ on \cref{alg:line:cl:add}.

\begin{algorithm}
  \caption{}
  \label{alg:generateNewCliques}
  \input{algorithms/generateNewCliques}
\end{algorithm}

\FunctionCall{mergeClique}{} merges the CoreGraphs to form a clique pattern graph. The algorithm starts similar to \cref{alg:mergecore:nonclique}. It generates the new pattern $np$ by connecting the marked vertex from $i$ ($u$) and its corresponding edges. Similarly, it joins a new vertex ($v$) which is the marked vertex in $j$ and its corresponding edges. To check if the graph is a clique, the algorithm takes a marked vertex from $c3$ and converts it to the Bliss space using \textbf{C} of $c3$. After applying the permutation $a2$ and converting it back to CoreGraph space, the algorithm uses the inverse canonical form of \textbf{I}. It converts the CoreGraph with $mv$ as the marked vertex. It then returns the generated clique pattern.

\subsubsection{Metric/Matcher Step}~\label{sec:matcher_step}

In graph mining, the standard practice often involves using metrics like \acf{mni} or MIS to determine if patterns occur frequently. We propose \ac{mal} as an alternative. What sets \ac{mal} apart is its ability to provide results without considering overlapped vertices or automorphisms while determining the occurrences of a particular pattern and hence having the ability to determine an independent set, thus preserving the fundamental integrity of the MIS metric. At the same time it can be completed as fast as a \ac{mni} metric. Additionally, our approach incorporates a slider, allowing users to fine-tune the degree of overlap in the results, giving them precise control over the output. It's essential to highlight that our method stands out due to its efficiency; unlike MIS, it avoids the NP-complete complexity; and unlike \ac{mni} it preserves the independent set property, making it a more practical and accessible tool for pattern analysis.

In this section, we first state the relationship between MIS and \ac{mal}. We then explain in detail about the proposed slider value and how to utilize it.

\paragraph{Comparison between Maximal and Maximum Independent Set}

We first start with deriving a relationship between the Maximum independent set and our metric \ac{mal}. 

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.66\linewidth}
      \centering
      \input{figures/diagram/malVisualizationDatagraph}
      \caption{Data graph $D_m$}
    \end{subfigure}
    \begin{subfigure}{0.33\linewidth}
      \centering
      \input{figures/diagram/malVisualizationPattern}
      \caption{Pattern graph $P_m$}
    \end{subfigure}
    \caption{Maximal independent set visualization}
    \label{fig:malVisual}
    \ifACM
      \Description{Maximal independent set visualization}
    \fi
\end{figure}

\begin{theorem}~\label{theo:mal}
  If $m$ is a maximal independent set, with the number of vertices in pattern graph $n$, and $M$ is a true maximum independent set, then $|M| \le |m|*n$.
\end{theorem}
Let us understand the \cref{theo:mal} with a simple example, as shown in \cref{fig:malVisual}.
In the figure, $D_m$ is the data graph and $P_m$ is the pattern graph $P$. 
According to MIS metric, $\set{u_1, u_2, u_3, u_4}$ would be mapped $\set{\set{d_1,d_2,d_3,d_4},\set{d_1,d_5,d_6,d_7},\set{d_2,d_8,d_9,d_{10}},\set{d_3,d_{11},d_{12},d_{13}},$\\$\set{d_4,d_{14},d_{15},d_{16}}}$. According to the definition of \ac{mal}, it can either pick the same embedding in which, the value of $|M|$ is $4$ and $|m|$ can be $1$ if $\is{\set{d_1,d_2,d_3,d_4}}$ are mapped.
Then $|m|*n$ would be $4$, which signifies we matched independent with one from each of MIS. So, in non-optimal matching $|M| = |m|*n$, otherwise $|M| < |m|*n$. Thus, substantiating our claim.

\cref{theo:mal} above gives an upper bound on the maximum independent set. We can rewrite the equation as $|M| / n \le |m|$. This is the lower bound of the effective support used in \ac{flexis}. In the next section, we use \ac{lerp} to adjust between the lower bound and upper bound of the effective support.

\paragraph{Slider}

In graph mining, various applications entail distinct requirements. For example, in network analysis, a degree of overestimation may be acceptable, whereas in fields like chemical composition analysis or biomedical research, precision is of paramount importance, even if it means potentially missing some patterns. To address these divergent needs, we introduce the Slider, a versatile metric designed to strike a balance. The Slider metric exhibits distinctive behavior based on the selected slider values. At a lower slider value, the Slider tends to exhibit an overestimation of pattern occurrences, and as the slider value increases, this overestimation gradually diminishes, eventually reaching zero at the highest threshold setting. However, at the highest threshold, \ac{flexis} can underestimate the pattern occurrences.

To provide a more precise perspective, our metric mirrors the performance of \ac{mni} at lower thresholds while getting close to MIS as the threshold value increases. This versatility grants users the flexibility to fine-tune the trade-off between accuracy and processing time, tailoring the metric to suit the specific needs of their applications. It is important to emphasize that our approach achieves performance levels akin to both \ac{mni} and MIS but at significantly reduced computational time, maintaining nearly equivalent accuracy when compared to traditional methods.

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=1.0\linewidth]{plots/logsliderpdf/p2p-Gnutella08-timeTaken}
        \caption{Time taken}
        \label{fig:slider:time}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=1.0\linewidth]{plots/logsliderpdf/p2p-Gnutella08-found}
        \caption{Frequent patterns}
        \label{fig:slider:frequent}
    \end{subfigure}
    \caption{Various slider values with Gnutella}
    \label{fig:slider:gnutella}
    \ifACM
      \Description{Various slider values with Gnutella}
    \fi
\end{figure}

Based on the proof of \cref{theo:mal}, which shows the relationship between the \ac{mal} and MIS, we define our slider value. 
According to the \cref{theo:mal}, $|M| \leq |m| * n$. If a pattern is frequent according to MIS with support \acs{support}, then $\sigma \leq |m| * n$. That means, $\sigma / n \leq |m|$. So, the lower threshold can be set to $\sigma / n$. Trivially, the upper threshold is \acs{support}.

\ac{flexis} calculates the threshold value $\tau$ using linear interpolation between $\frac{\sigma}{n}$ and \acs{support}. $\ac{lerp}$ represents a value within the range of [0.0, 1.0], and is employed to determine the point along the line formed by the lower and higher thresholds. 
If the pattern occurrences are over the effective threshold $\tau$, we deem it frequent.
We can write an equation for this $\tau = \sigma (1 - 1/n) \lambda + \sigma / n$, where $\lambda$ is the slider.
With $\sigma=600$ and $\lambda=0.4$, we get $420, 360,$ and $330$ for size-2, size-3 and size-4 patterns. Thus a pattern will be considered frequent if it occurs over $\tau$ times rather than \acs{support} times.

We show the time taken (\cref{fig:slider:time}) and the number of frequent patterns (\cref{fig:slider:frequent}) for varied values of $\ac{lerp}$.
As expected, the number of patterns found decreases with increase in $\ac{lerp}$, because of reduction in overestimation. Also, the time required to find the patterns decrease with increase in $\ac{lerp}$, as the number of patterns searched for decreases.

\begin{algorithm}
  \caption{vf3Matching}
  \label{alg:matching}
  \input{algorithms/vf3matcher}
\end{algorithm}

\paragraph{Extensions to VF3Light}

\ac{flexis} adapts vf3Light~\cite{carletti:2018:vf3, carletti:2019:vf3} for matching pattern graphs in a data graph. To achieve maximal independent set of data vertices given the pattern graphs, we extended the \FunctionCall{MatchingEngine}{}, \FunctionCall{VF3LightSubState}{}, and \FunctionCall{MatchingVisitor}{}.

\paragraph{MatchingEngine}
VF3Light uses \FunctionCall{MatchingEngine}{} to compute subgraph isomorphism.
\ac{flexis} modifies \FunctionCall{MatchingEngine}{} to \FunctionCall{MiningMatchingEngine}{} which overrides the \FunctionCall{FindAllMatchings}{} function.

\begin{algorithm}
  \caption{FindAllMatchings}
  \label{alg:matching:findAllMatching}
  \input{algorithms/findAllMatching}
\end{algorithm}

The \cref{alg:matching:findAllMatching} shows the function for computing maximal independent set matching given a datagraph. VFState is the struct used by VF3 to store data graph, pattern graph, threshold, and other intermediate data such as which data vertex is mapped to which pattern vertex. We added a new a function \FunctionCall{MiningPossible}{} which checks if the candidate data vertex is unused. We also modified matchingEngine to set a boolean flag for early exit from current recursion stack (\cref{alg:matching:findAllMatching} \cref{line:findAllMatching:cf1}, \cref{line:findAllMatching:cf2},\cref{line:findAllMatchingRec:cf3},\cref{line:findAllMatchingRec:cf4}) if a match is found.


% \paragraph{VF3LightSubState}
\ac{flexis} extends the matching functionality VF3LightSubState to encompass mining via VF3LightMining. The substate is an extension of VFState, which we extended to also store intermediate data for used data vertices bitmap (used), num of instances found (count) and threshold (threshold). These variables are shared across different instances of VFState for the same pattern graph to avoid expensive copies.


% \paragraph{MatchingVisitor}
VF3Light provides a visitor interface that is passed to the matching engine as referenced in \cref{alg:matching:visitor}. Upon each discovery of a match by VF3Light, this function is invoked. The function serves to both increment the count and set the bitmap of the associated utilized vertices. The value returned by this function plays a crucial role in determining whether the matching engine should cease its search for new matches.

\begin{algorithm}
  \caption{visitor}
  \label{alg:matching:visitor}
  \input{algorithms/visitor}
\end{algorithm}

\subsection{Proofs for propositions}

  \begin{proof}[Proof for \cref{lemma:nAV}]
  According to our assumption the graph considered is not a clique. For a non-clique graph, the diameter is at least $2$ (trivial from the definition of diameter).
  
  According to Lemma~\ref{lemma:dia}, for any connected graph with more than 2 vertices, there are at least two vertices that are \ac{nav} and have their distance equivalent to the diameter of the graph.
  
  Hence, there is at least two \ac{nav} that have a distance of at least $2$ from each other. Thus, these two \ac{nav} must not have an edge between them.
  
  \end{proof}
  
  
  \begin{proof}[Proof for \cref{lemma:candidateGeneration}]
    \acf{flexis} generates $k$-size candidate pattern graph by merging 2 $(k-1)$-size frequent patterns on non-articulation vertices that do not have an edge between them when their CoreGraph is the same. To prove all candidate patterns can be generated, we need to prove the completeness and uniqueness of the candidate pattern generation method.
  
    The uniqueness of the candidate pattern generation method is trivial, as all the permutations are considered and the automorphism is removed. Thus, we only need to prove the completeness of the candidate pattern generation method.
  
    We can prove this via contradiction. That is, we assume that all candidate patterns cannot be generated by combining 2 $(k-1)$-size frequent patterns on the non-articulation vertices. Then there, exists a $(k)$-size pattern that can be formed by only combining 2 $(k-1)$-size patterns on the articulation vertices. Then, all the vertices of the $(k)$-size pattern must be articulation vertices. This is a contradiction according to Lemma~\ref{lemma:nAV}, and since cliques are generated separately we can assume that the graph is not a clique.
  \end{proof}
  
\begin{proof}[Proof for \cref{theo:candidateGeneration}]
  We can prove this via induction. For the base case of $k=2$, we consider all the possible edges in the data graph. Thus, by definition of \ac{flexis} all the $2$-size candidate patterns can be generated. To prove that every non-clique candidate pattern can be generated, we show that if all the frequent patterns of size $k-1$ can be generated, then all the candidate patterns of size $k$ can be generated, as shown in \cref{lemma:candidateGeneration}. Thus, by induction, we can prove that all the candidate patterns can be generated.
\end{proof}

\begin{proof}[Proof for \cref{theo:mal}]
  We prove this via contradiction. Assume for the sake of contradiction that the proposed condition is not true, i.e., $|M| > |m|*n$.
  Since, $|M| > |m|*n$, we have more embeddings in $|M|$ than vertices in $m$. This means there is at least one independent set in $M$ that must not have any of the $|m|*n$ vertices of $m$. Hence $M$ has an embedding $E$ which does not have any vertex in $m$, which makes it possible to insert $E$ into $m$ and produce a larger independent set. This violates $m$ being a maximal independent set. Hence, a contradiction is found and $|M| \leq |m| * n$.
\end{proof}

\section{Results}~\label{sec:results}

In this section, we evaluate \ac{flexis} and compare it with GraMi and T-FSM. For this we utilize the code provided by the authors for GraMi and T-FSM. The original version of GraMi uses java 17.0.7 and T-FSM uses C++. We implement our method in C++ compiled by g++\-11. We ran our experiments on Xeon CPU E5-4610 v2 (2.30GHz) on Ubuntu 22.04. Our system has 192 GB DDR3 memory.

\textbf{Datasets}
We use $5$ real-world graph dataset with varied number of vertices, edges and labels. The datasets included are as follows, 
\begin{enumerate}
    \item Gnutella08~\cite{leskovec:2007:graph, ripeanu:2002:mapping} constitutes a specific instance captured from the Gnutella peer-to-peer file sharing network.
    \item The soc-Epinions1~\cite{richardson:2003:trust} is derived from online social network Epinions.com, a consumer review website. 
    \item The Slashdot~\cite{leskovec:2009:community}reveals user interconnections on Slashdot's tech news platform. 
    \item The wiki-vote dataset~\cite{leskovec:2010:signed, leskovec:2010:predicting} is a compilation of voting interactions within Wikipedia.
    \item MiCo~\cite{elseidy:2014:grami} dataset is Microsoft co-authorship information.
\end{enumerate}

\cref{tab:datasets} shows the properties of these data graphs. $|V_d|$ refers to the maximum degree of the graph, $|V_l|$ is the number of distinct vertex labels, and $|E_l|$ is the number of distinct edge labels. Vertex and edge labels are randomly assigned to vertices and edges, respectively. 

\begin{table}
  \caption{Datasets used for experiments}
  \label{tab:datasets}
  \input{tabular/datasets}
\end{table}

\textbf{Metrics}
The support threshold \acs{support}, in conjunction with a given data graph, serves as the input for the proposed system. The assessment of our system encompasses the execution time incurred during the mining process, analysis on the frequent pattern obtained, and the quantification of memory utilization. We compare our method to both the modifications of the state-of-art algorithm GraMi, namely the AGrami,  where $\alpha$ is set to $1$, and the baseline GraMi version. We also compare our algorithm with the newest graph mining system T-FSM. In T-FSM we compare our method with both the \ac{mni} version and the fractional score version. Conversely, for our developed algorithm denoted as \ac{flexis}, we present two distinct variants. The first variant entails an implementation absent of any approximation mechanisms. In contrast, the second variant pursues the generation of maximal frequent patterns, a subset of which intersects optimally with those identified by GraMi and T-FSM. Since, the problem can run for a long time in case of large graphs, we restrict the time that both the algorithms run to 30 mins, after which the system times out. If an algorithm times out then the corresponding values will be missing in the graphs. 

\subsection{Methodology}
It is commonly known that the number of times a pattern occurs is overestimated by \ac{mni} and as a consequence the number of patterns classified as frequent is more than the actual value for GraMi. And a similar explanation also holds for Tfsm-MNI. If we take a closer look at the functioning of Tfsm using fractional-score, there is still a considerable over-estimation. However, this over-estimation is much less than that of GraMi. 

In contrast, our method spans from over-estimating to under-estimating, with over-estimation happening at a lower \ac{lerp} value and under-estimation possibly at a higher value. Thus, we postulate that we will merge closer to GraMi at a lower value of \ac{lerp}, to the T-FSM-MNI at a similar value and to T-FSM-fractional, at the same or higher value, depending on the efficiency of fractional-score with those datasets. From our experiments, as shown in the graph \cref{fig:log:TimeTaken:Gnutella} most of the values of execution time of Tfsm-Frac (lowest among the other comparing methods) falls closer to our slider value of 0.5 and most of the values are a little above the slider value of 0.5. Also, as can be seen in the \cref{tab:similarity} the number of frequent pattern in all the three algorithms, namely \ac{flexis}, GraMi and T-FSM merge at 0.4. Thus, we choose slider value of 0.4 as the apt one for comparison.

Our method uses a undirected data loader and a directed matching algorithm. Thus, to determine the effciency of performance, only looking at the undirected version might not be fair. Since GraMi has both undirected and directed version we choose to consider the directed version of GraMi. Moreover T-FSM proposes a better undirected version of GraMi with some optimisations. Thus, instead of considering the original undirected GraMi we use the T-FSM version of GraMi, referred to as T-FSM MNI. We also compare our algorithm with T-FSM fractional score model. It is important to note that our observations between GraMi and T-FSM does not follow directly from their paper. This is because we consider directed GraMi, while their paper considered the undirected version. Also, since the paper itself postulated the equivalent performance of their \ac{mni} version with that of GraMi and better performance of their fractional-score method when compared to GraMi, we do not reinforce this point again in this paper, rather here we use their important observations.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{plots/logGnutellaPdf/p2p-Gnutella08-timeTaken}
    \caption{Gnutella}
    \label{fig:log:TimeTaken:Gnutella}
    \ifACM
      \Description{Plots for execution time}
    \fi
    \vspace{-10pt}
\end{figure}

\begin{figure*}[htb]
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/mico-timeTaken}
    \caption{MiCo}
  \end{subfigure}
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/soc-Slashdot0902-timeTaken}
    \caption{Slashdot}
  \end{subfigure}
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/wiki-Vote-timeTaken}
    \caption{wiki-Vote}
  \end{subfigure}
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/soc-Epinions1-timeTaken}
    \caption{Epinions}
  \end{subfigure}

  \caption{Execution Time}
  \label{fig:log:TimeTaken}
  \ifACM
    \Description{Plots for execution time}
  \fi
\end{figure*}

\begin{figure*}[htb]
  \centering
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/p2p-Gnutella08-memoryUsed}
    \caption{Gnutella}
  \end{subfigure}
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/soc-Slashdot0902-memoryUsed}
    \caption{Slashdot}
  \end{subfigure}
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/wiki-Vote-memoryUsed}
    \caption{wiki-Vote}
  \end{subfigure}
  \begin{subfigure}{0.245\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/soc-Epinions1-memoryUsed}
    \caption{Epinions}
  \end{subfigure}

  \caption{Memory Usage}
  \label{fig:log:MemoryUsage}
  \ifACM
    \Description{Plots for memory usage}
  \fi
\end{figure*}

\begin{figure*}[htb]
  \centering
  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/p2p-Gnutella08-found}
    \caption{Gnutella}
    \label{fig:log:freq:Gnu}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/soc-Slashdot0902-found}
    \caption{Slashdot}
    \label{fig:log:freq:dot}
  \end{subfigure}

  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/p2p-Gnutella08-searched}
    \caption{Gnutella}
    \label{fig:log:srch:Gnu}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=1.0\linewidth]{plots/logpdf/soc-Slashdot0902-searched}
    \caption{Slashdot}
    \label{fig:log:srch:dot}
  \end{subfigure}
  
  
  
  
  
  
  
  
  
  
  \caption{Frequent (a, b) and Searched (c, d) Patterns}
  \label{fig:log:FrequentSearched}
  \ifACM
    \Description{Plots for frequent and searched patterns}
  \fi
\end{figure*}

\subsection{Computation of Frequent Subgraphs}

We evaluate the performance of \ac{flexis}, GraMi, and T-FSM in terms of the time taken to compute frequent subgraphs. The outcomes of both systems were recorded, with a predetermined time limit of $30$ minutes. For the sake of clarity, we denote GraMi as \qoutes{GraMi}, while numeric identifiers are used for different configurations of \ac{flexis} \cref{fig:log:TimeTaken}. T-FSM fusion based algorithm is shown as \qoutes{TfsmFrac} while T-FSM \ac{mni} is shown as \qoutes{TfsmMNI}. \ac{flexis} is characterized by a parameter range spanning $\left[0.0, 1.0\right]$ (\ac{lerp}), where $0.0$ corresponds to the fraction $\ac{mal}$ and $1.0$ corresponds to \acs{support}, while intermediate values are derived through linear interpolation.

Execution Time for Gnutella dataset, across varied slider values, along with GraMi and T-FSM is as shown in \cref{fig:log:TimeTaken:Gnutella}.For MiCo, Epinions, Slashdot, and wiki-Vote datagraphs in \cref{fig:log:TimeTaken}. 
Across Epinions, Slashdot and wiki-Vote, slider $0.4$ performs with average speed up of 3.02x over T-FSM fractional and 10.58x over GraMi.
While with Gnutella, slider $0.4$ with average speed up of 1.97x over T-FSM fractional and 7.90x over GraMi.
Notably, the number of frequent subgraphs exhibits a growth pattern as the support value is decreased.

\subsection{Memory Usage} \label{sec:results:memoryUsage}
\Cref{fig:log:MemoryUsage} presents memory utilization patterns observed during the processing of the Epinions and wiki-Vote datagraphs by both \ac{flexis}, GraMi and T-FSM. It is important to note that instances where execution was prematurely terminated due to reaching predefined timeout constraints do not have corresponding memory utilization values represented.
Significantly, discernible differences in memory utilization patterns emerge between the three systems due to their distinct storage strategies. Specifically, GraMi maintains an expansive repository of both frequent and infrequent graphs, hence higher memory demand.
Similarly, T-FSM is build on top of GraMi has similar memory requirements, but it has efficient usages compared to GraMi.
T-FSM takes all the candidate patterns and does a memory bounded search in the datagraph, which leads to lower memory requirement.
On the contrary, \ac{flexis} exhibits a discerning approach by conserving solely the frequent graphs at each level. Notably, when the potential for the creation of $k+1$ vertices arises, our method exclusively retains the prevalent $k$-vertices, thereby adapting a more resource-efficient memory management framework.

In the \cref{fig:log:MemoryUsage}, GraMi and T-FSM Fractional uses 8.79x and 1.01x memory than \ac{flexis} ($\lambda = 0.4$) in average across wiki-Vote, Epinions, and Slashdot. With the addition of Gnutella GraMi and T-FSM Fractional uses 5.83x and 0.64x more memory than \ac{flexis}. \ac{flexis} searches more than both the frameworks in Gnutella dataset. This leads to higher number of frequent and searched patterns.

We can also observe, as the support value decreases, the memory utilization proportionately increases. This phenomenon occurs due to the greater number of patterns being recognized as frequent as the support threshold decreases. This trend is consistent across both GraMi and our method \ac{flexis}. In the context of our approach, a reduction in the \ac{lerp} value corresponds to an elevated count of frequent patterns, consequently translating to an increase in memory requirement. It is crucial to acknowledge that this increased memory allocation, with decrease in support, in our approach is essential, as the nature of the mining problem necessitates the retention of identified frequent subgraphs. In stark contrast to GraMi, our approach refrains from incurring any excess memory overhead beyond that required to store the indispensable patterns. Thus, our approach effectively harnesses considerably less memory in comparison to GraMi. While in comparison to T-FSM, \ac{flexis} sometimes have higher memory consumption (Gnutella and MiCo), while other times ours more efficient (Epinions, Slashdot, and wiki-Vote). This is because the memory utilisation reported is the maximum utilisation and it is possible that at a particular time in the entire process we might have had a slightly higher memory utilisation.

\subsection{Frequent Subgraph Instances}
The graphs shown in \cref{fig:log:srch:Gnu} and \cref{fig:log:srch:dot} demonstrate that we conducted fewer pattern searches compared to the GraMi and T-FSM algorithm.
\ac{flexis} searches more candidate patterns as the effective threshold $\tau$ reduces as $\lambda$ decreases. \ac{flexis} ($\lambda=0.4$) searches 7.2x and 5.7x more than GraMi and T-FSM fractional.
Our method was able to find patterns that were almost as common as those found by GraMi and T-FSM, as shown in \cref{fig:log:freq:Gnu} and \cref{fig:log:freq:dot}.
On average \ac{flexis}($\lambda=0.4$)  found 8.8x and 2.4x more than frequent patterns than GraMi and T-FSM fractional.
To show that these patterns are similar, we used graph isomorphism, and the results are as shown in \cref{tab:similarity}. In the table, $f_g, f_f, f_t$ refers to frequent patterns generated by GraMi, \ac{flexis}, and T-FSM respectively. We show only for one dataset because of the lack of space. 

\begin{table}[htb]
    \centering
    \caption{Similarity with \ac{flexis} $\lambda = 0.4$ on Epinions}
    \label{tab:similarity}
    \input{tabular/similarity}
\end{table}

As can be noticed, there is not a complete intersection between both, this can be attributed to the following reasons,
\begin{itemize}
    \item \textbf{Difference in the approach:} Our method uses an undirected data processing and directed matcher method, while GraMi uses fully directed search. So there is a possibility that we are getting some pattern that are frequent, which GraMi does not find.
    \item \textbf{Difference in over-estimation:} In lower slider values, \ac{mal} tends to over-estimate due to the approximation applied to the threshold value. In contrast, the over-estimation of GraMi is due to recounting of the same vertices, considering automorphism and so on. Thus, the over-estimated patterns might not match between \ac{mal} and GraMi.
\end{itemize}

The reason we conducted fewer searches is because of our smart way of choosing which patterns to look for.
We focused only on exploring graphs that could be made from the frequent graphs we found earlier.
In contrast, we didn't spend time looking at all the possible extensions that could come from the frequent graphs in previous steps, which is how GraMi works.

\subsection[FLEXIS slider]{FLEXIS $\lambda$}
We experimented \ac{flexis} with different \ac{lerp} value. $1.0$ \ac{lerp} means no approximation and $0.0$ means all the frequent patterns which satisfy $\frac{\sigma}{\abs{V_p}}$. We emphersize on the results produced by $0.4$ as it most closely have same characteristics as GraMi, in terms of number of patterns graphs being searched. While searching in a similar search space, we more pattern graphs due to lower effective threshold $\tau$. However, we generate only better candidate pattern generation.

\section{Related Work}~\label{sec:related}

The solution to the FSM problem can be largely derived from a two-step process, primarily extended from the work of ~\cite{nguyen:2022:subgraph}. The initial step, referred to as the \sqoutes{Generation step}, involves the creation of all possible candidate patterns and potential subgraph candidates. Following this, the candidate subgraph space is streamlined by pruned automorphisms. Lastly, the \sqoutes{Metric step} is the number of isomorphic instances among the selected candidates within the data graph, determining whether it exceeds a predefined support. Many of the algorithms presented in the context of Subgraph Isomorphism focus on modifying one or more of these components to enhance overall performance.

In the generation step, all possible subgraphs can be achieved through two main methods: edge extension and vertex extension. In the edge extension methods, a candidate subgraph is derived from an existing frequent candidate by adding an edge. This process can be accomplished in two distinct ways. Initially, the path extension approach is employed, where vertices within the frequent subgraph are expanded by adding edges, as illustrated in previous works such as Peregrine, GSpan, Pangolin, and Arabesque~\cite{jamshidi:2020:peregrine,yan:2002:gspan,chen:2020:pangolin, teixeira:2015:arabesque}. Alternatively, the utilization of level-wise methods becomes prominent, wherein two frequent subgraphs of order $k$ combine to form a subgraph of order $k+1$~\cite{kuramochi:2005:finding}. In the context of vertex extension methods, the frequent subgraphs are expanded by adding a vertex~\cite{chen:2020:pangolin, teixeira:2015:arabesque}. Notably, there has been limited exploration into the extension of level-wise notions within the context of vertex extension scenarios. In this paper, we introduce a novel approach that integrates the level-wise methodology into vertex extension methods.  

Within the generation step, the redundant and automorphic candidate graphs must be eliminated. The common practice involves the utilization of canonical representations to eliminate redundant candidate graphs that are generated. Diverse canonical representations exist, including the Minimum DFS Code representation~\cite{yan:2002:gspan}, Bliss~\cite{junttila:2007:engineering}, Eigen Value representations~\cite{zhao:2020:kaleido}, Canonical Adjacency matrix representations, as well as Breadth First Canonical String and Depth First Canonical String representations~\cite{jiang:2013:survey}, among others. Given its exceptional efficiency, Bliss is selected as the method of choice in this paper.

The last step of FSM is the 'Metric' phase, wherein the generated candidates are compared with the data graphs to ascertain the frequency of occurrence (matches) of a specific candidate within the data graph. This comparison also involves assessing whether the match count exceeds a predefined threshold. Subgraph isomorphism methods are employed for match determination. Varied iterations of this phase exist within the literature. The gold standard is utilizing the Maximum Independent Set~\cite{fiedler:2007:support}, which identifies the maximal number of disjoint subgraph isomorphisms in the primary graph, an NP-complete problem in itself. An alternative, SATMargin~\cite{liu:2022:satmargin}, employs random walks, framing the subgraph mining challenge as a SAT problem and employing a SAT algorithm (such as CryptoMiniSat~\cite{soos:2019:cryptominisat}) for its resolution. Notably, the most prevailing approximation method is \ac{mni}~\cite{bringmann:2008:frequent}, which tends to overestimate the number of isomorphic patterns by allowing certain overlaps. \ac{mni} finds extensive utilization either directly or with subsequent optimization strategies~\cite{elseidy:2014:grami,jamshidi:2020:peregrine,chen:2020:pangolin,chen:2021:sandslash}. In the context of GraMi~\cite{elseidy:2014:grami}, graph mining is conceptualized as a Constraint Satisfaction Problem (CSP) that uses \ac{mni} to prune the search space. Other metrics that are an extension to \ac{mni}, such has fractional score, which alleviates the over-estimation of \ac{mni} have also been proposed~\cite{yuan:2023:tfsm}. While this method succeeds in reducing the over-estimation to a limit, it still shows a substantial overestimation. Therefore, this paper introduces an innovative metric termed 'Maximal Independent Set,' an approximation of the Maximum Independent Set that provides the users with a slider to control the overlap that is required with the Maximum Independent set. While we might also overestimate, it can be brought to the minimum if the user chooses so. Notably, our proposed method diverges from the concepts of maximal frequent subgraph as discussed in SATMargin~\cite{liu:2022:satmargin} and Margin~\cite{thomas:2010:margin}, wherein the focus is on determining the maximum feasible size of a frequent subgraph, as opposed to utilizing it as a metric, as shown in our study.

While tangential to the core focus of this paper, the subsequent passages are included to provide a definitive categorization of our study.

FSM algorithms can be classified into two distinct categories: 1) Transactional methods, and 2) Single-graph methods. Transactional algorithms~\cite{liu:2022:satmargin, thomas:2010:margin}, define a frequent pattern as one that occurs across a set number of graphs. In other words, within a collection of $N$ data graphs, a pattern is deemed frequent if it emerges in more than \ac{support} data graphs. Conversely, the single graph paradigm considers a pattern frequent if it repeats a predefined number of times within a single large graph~\cite{elseidy:2014:grami, nguyen:2021:method, mawhirter:2021:graphzero, jamshidi:2020:peregrine, chen:2022:efficient}. This paper squarely falls within the realm of Single-graph methods. Notably, there exist other methodological extensions within FSM that aim to ascertain precise support counts~\cite{nguyen:2020:fast}, solely consider closed-form solutions~\cite{nguyen:2021:method}, or delve into weighted subgraph mining~\cite{le:2020:mining}. These extensions, however, lie outside the scope of our current investigation.

Moreover, Subgraph Mining can be achieved through diverse ways, spanning CPU-based approaches~\cite{elseidy:2014:grami, mawhirter:2019:automine, mawhirter:2021:graphzero, aberger:2017:emptyheaded, shi:2020:graphpi, jamshidi:2020:peregrine}, GPU-accelerated techniques~\cite{chen:2020:pangolin, guo:2020:gpu, guo:2020:exploiting, chen:2022:efficient}, Distributed Systems~\cite{salem:2021:rasma}, near-memory architectures~\cite{dai:2022:dimmining}, and out-of-core systems~\cite{zhao:2020:kaleido}. In this present study, we focus exclusively on CPU-based architectures. However, it is important to note that our proposed method exhibits adaptability for potential extension to GPU and other architectural frameworks.

\section{Conclusion}~\label{sec:conclusion}
In this paper, we introduce a novel metric based on maximal independent sets (MIS) that enables users to fine-tune the level of overlap they require with the original results. This level of customizability can be invaluable, particularly in applications where precision is paramount. We also proposed an innovative technique for efficiently generating the candidate search space by merging previously identified frequent subgraphs. This approach significantly reduced the computational overhead associated with graph mining, making it more accessible and practical. By incorporating these methods we showed that our method performs better than the existing state-of-art GraMi and T-FSM. In essence, our contributions pave the way for more effective and versatile graph mining techniques, expanding their utility across a wide spectrum of applications.



==> figures/articulation.tex <==
\begin{tikzpicture}
  \node[redNode] (d1) at (0, 0) {$d_1$};
  \node[redNode] (d2) at (1.0, 0) {$d_2$};
  \node[redNode] (d3) at (2.0, 0.5) {$d_3$};
  \node[redNode] (d4) at (3.0, 0) {$d_4$};

  \node[blueNode] (d5) at (0, 1.0) {$d_5$};
  \node[blueNode] (d6) at (1.0, 1.0) {$d_6$};
  \node[blueNode] (d7) at (3.0, 1.0) {$d_7$};

  \draw[doubleArrow] (d1) -- (d2);
  \draw[doubleArrow] (d1) -- (d5);
  \draw[doubleArrow] (d5) -- (d6);

  \draw[doubleArrow] (d2) -- (d3);
  \draw[doubleArrow] (d6) -- (d3);

  \draw[doubleArrow] (d3) -- (d7);
  \draw[doubleArrow] (d3) -- (d4);
\end{tikzpicture}


==> figures/articulation1.tex <==
\begin{tikzpicture}
  \node[redNode] (d1) at (0, 0) {$d_1$};
  \node[redNode] (d2) at (1, 0) {$d_2$};
  \node[redNode] (d3) at (2, 0.5) {$d_3$};

  \node[blueNode] (d5) at (0, 1) {$d_5$};
  \node[blueNode] (d6) at (1, 1) {$d_6$};

  \draw[doubleArrow] (d1) -- (d2);
  \draw[doubleArrow] (d1) -- (d5);
  \draw[doubleArrow] (d5) -- (d6);

  \draw[doubleArrow] (d2) -- (d3);
  \draw[doubleArrow] (d6) -- (d3);
\end{tikzpicture}


==> figures/articulation2.tex <==
\begin{tikzpicture}
  \node[redNode] (d3) at (1, 0.5) {$d_3$};
  \node[redNode] (d4) at (2, 0) {$d_4$};

  \node[blueNode] (d7) at (2, 1) {$d_7$};

  \draw[doubleArrow] (d3) -- (d7);
  \draw[doubleArrow] (d3) -- (d4);
\end{tikzpicture}


==> figures/core/core2u1.tex <==
\begin{tikzpicture}
  \node[markedNode] (u1) at (0, 0) {$u_1$};
  \node[blueNode] (u2) at (1.3, 0) {$u_2$};
  \node[blueNode] (u4) at (1.3, 1.3) {$u_4$};
  \draw[doubleArrow] (u2) -- (u4);
\end{tikzpicture}


==> figures/core/core2u2.tex <==
\begin{tikzpicture}
  \node[redNode] (u1) at (0, 0) {$u_1$};
  \node[markedNode] (u2) at (1.3, 0) {$u_2$};
  \node[blueNode] (u4) at (1.3, 1.3) {$u_4$};
  \draw[doubleArrow] (u1) -- (u4);
\end{tikzpicture}


==> figures/core/core2u4.tex <==
\begin{tikzpicture}
  \node[redNode] (u1) at (0, 0) {$u_1$};
  \node[blueNode] (u2) at (1.3, 0) {$u_2$};
  \node[markedNode] (u4) at (1.3, 1.3) {$u_4$};
  \draw[doubleArrow] (u1) -- (u2);
\end{tikzpicture}


==> figures/runningDatagraph.tex <==
\begin{tikzpicture}

  \def\smallerScale{18}
  \def\biggerScale{22}
  \def\smallerWidth{4}
  \def\biggerWidth{6}

  \node[redNode] (d1) at (-1.5, 0) {$d_1$};
  \node[redNode] (d2) at (-0.5, 0) {$d_2$};
  \node[redNode] (d3) at (0.5, 0) {$d_3$};
  \node[redNode] (d4) at (1.5, 0) {$d_4$};

  \node[blueNode] (d5) at (-1.0, 1.0) {$d_5$};
  \node[blueNode] (d6) at (0, 1.0) {$d_6$};
  \node[blueNode] (d7) at (1.0, 1.0) {$d_7$};

  \draw[doubleArrow] (d1) -- (d2);
  \draw[doubleArrow] (d2) -- (d3);
  \draw[doubleArrow] (d3) -- (d4);

  \draw[doubleArrow] (d5) -- (d6);
  \draw[doubleArrow] (d6) -- (d7);

  \draw[doubleArrow] (d1) -- (d5);
  \draw[doubleArrow] (d2) -- (d5);

  \draw[doubleArrow] (d2) -- (d6);
  \draw[doubleArrow] (d3) -- (d6);

  \draw[doubleArrow] (d3) -- (d7);
  \draw[doubleArrow] (d4) -- (d7);

  \begin{scope}[on background layer]
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d1) {};
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d5) {};
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d2) {};
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d1) -- (d5);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d2) -- (d5);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d2) -- (d1);
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d3) {};
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d4) {};
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d7) {};
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d3) -- (d4);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d7) -- (d4);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d7) -- (d3);

    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d3) {};
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d6) {};
    \node[circularNode, fill=blue!40, scale=\biggerScale] at (d2) {};
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d3) -- (d6);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d2) -- (d6);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d2) -- (d3);
    \draw[singleEdge, fill=blue!40, draw=blue!40, line width=\biggerWidth] (d7) -- (d3);
  \end{scope}

\end{tikzpicture}


==> results/eecs1.30m/artifacts/plotTable/tex/p2p-Gnutella08.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
100 & GraMi & 125 & 6825 & 145.102000 & 1336.214844 \\
100 & 1.0 & 120 & 6016 & 1.222000 & 50.200000 \\
50 & GraMi & 276 & 14726 & 380.759000 & 1626.503906 \\
50 & 1.0 & 139 & 6567 & 1.522000 & 53.712000 \\
\bottomrule
\end{tabular}


==> results/eecs1.30m/artifacts/plotTable/tex/soc-Epinions1.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
8000 & GraMi & 0 & 125 & 2.297000 & 824.066406 \\
8000 & 1.0 & 0 & 450 & 2.050000 & 61.448000 \\
4000 & GraMi & 0 & 125 & 16.648000 & 1004.457031 \\
4000 & 1.0 & 0 & 450 & 1.670000 & 61.348000 \\
3000 & GraMi & 0 & 125 & 15.346000 & 1035.773438 \\
3000 & 1.0 & 0 & 450 & 2.002000 & 61.424000 \\
1000 & 1.0 & 100 & 4550 & 17.506000 & 67.620000 \\
\bottomrule
\end{tabular}


==> results/eecs1.30m/artifacts/plotTable/tex/soc-Slashdot0902.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
8000 & GraMi & 0 & 125 & 45.490000 & 1726.101562 \\
8000 & 1.0 & 0 & 450 & 2.941000 & 97.864000 \\
4000 & GraMi & 0 & 125 & 46.795000 & 1147.757812 \\
4000 & 1.0 & 0 & 450 & 3.014000 & 97.852000 \\
3000 & 1.0 & 0 & 450 & 3.145000 & 97.872000 \\
\bottomrule
\end{tabular}


==> results/eecs1.30m/artifacts/plotTable/tex/test10.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
2 & GraMi & 19 & 70 & 0.159000 & 59.101562 \\
2 & 1.0 & 9 & 52 & 0.003000 & 5.288000 \\
1 & GraMi & 484 & 2596 & 2.420000 & 596.160156 \\
1 & 1.0 & 313 & 2836 & 0.429000 & 40.188000 \\
\bottomrule
\end{tabular}


==> results/eecs1.30m/artifacts/plotTable/tex/wiki-Vote.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
700 & GraMi & 0 & 125 & 0.274000 & 197.628906 \\
700 & 1.0 & 0 & 447 & 0.204000 & 14.172000 \\
600 & GraMi & 0 & 125 & 0.285000 & 196.578125 \\
600 & 1.0 & 0 & 447 & 0.204000 & 14.152000 \\
500 & GraMi & 0 & 125 & 0.333000 & 191.421875 \\
500 & 1.0 & 0 & 447 & 0.203000 & 14.192000 \\
400 & GraMi & 0 & 125 & 2.005000 & 210.796875 \\
400 & 1.0 & 0 & 447 & 0.203000 & 14.176000 \\
300 & GraMi & 91 & 4197 & 82.885000 & 1382.359375 \\
300 & 1.0 & 0 & 447 & 0.206000 & 14.212000 \\
200 & 1.0 & 95 & 4089 & 1.745000 & 38.260000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plot/tex/p2p-Gnutella08.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
100 & GraMi & 125 & 6825 & 84.058000 & 507.472656 \\
100 & 1.0 & 120 & 6016 & 0.725000 & 50.100000 \\
90 & GraMi & 125 & 6825 & 91.347000 & 532.960938 \\
90 & 1.0 & 125 & 6500 & 0.769000 & 53.600000 \\
80 & GraMi & 125 & 6825 & 94.229000 & 503.812500 \\
80 & 1.0 & 125 & 6500 & 0.772000 & 53.604000 \\
70 & GraMi & 125 & 6825 & 98.261000 & 520.980469 \\
70 & 1.0 & 125 & 6500 & 0.778000 & 53.560000 \\
60 & GraMi & 129 & 6932 & 96.405000 & 536.621094 \\
60 & 1.0 & 125 & 6500 & 0.774000 & 53.604000 \\
50 & GraMi & 276 & 14726 & 222.601000 & 648.355469 \\
50 & 1.0 & 139 & 6567 & 0.783000 & 53.616000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plot/tex/soc-Epinions1.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
8000 & GraMi & 0 & 125 & 1.079000 & 875.867188 \\
8000 & 1.0 & 0 & 450 & 1.392000 & 61.340000 \\
7000 & GraMi & 0 & 125 & 1.395000 & 812.457031 \\
7000 & 1.0 & 0 & 450 & 1.394000 & 61.304000 \\
6000 & GraMi & 0 & 125 & 1.073000 & 827.636719 \\
6000 & 1.0 & 0 & 450 & 1.398000 & 61.312000 \\
5000 & GraMi & 0 & 125 & 1.009000 & 772.367188 \\
5000 & 1.0 & 0 & 450 & 1.398000 & 61.248000 \\
4000 & GraMi & 0 & 125 & 10.237000 & 955.480469 \\
4000 & 1.0 & 0 & 450 & 1.863000 & 61.352000 \\
3500 & GraMi & 0 & 125 & 10.031000 & 955.500000 \\
3500 & 1.0 & 0 & 450 & 1.390000 & 61.272000 \\
3000 & GraMi & 0 & 125 & 10.275000 & 1024.406250 \\
3000 & 1.0 & 0 & 450 & 1.392000 & 61.340000 \\
2500 & GraMi & 0 & 125 & 10.325000 & 1039.921875 \\
2500 & 1.0 & 0 & 450 & 1.856000 & 61.268000 \\
2000 & GraMi & 0 & 125 & 10.406000 & 993.640625 \\
2000 & 1.0 & 0 & 450 & 1.395000 & 61.304000 \\
1500 & 1.0 & 0 & 450 & 1.393000 & 61.256000 \\
1000 & 1.0 & 100 & 4550 & 13.321000 & 67.520000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plot/tex/soc-Slashdot0902.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
8000 & GraMi & 0 & 125 & 27.305000 & 1715.941406 \\
8000 & 1.0 & 0 & 450 & 2.386000 & 97.716000 \\
7000 & GraMi & 0 & 125 & 28.134000 & 1877.316406 \\
7000 & 1.0 & 0 & 450 & 2.388000 & 97.768000 \\
6000 & GraMi & 0 & 125 & 29.227000 & 1590.371094 \\
6000 & 1.0 & 0 & 450 & 2.371000 & 97.676000 \\
5000 & GraMi & 0 & 125 & 29.733000 & 1858.261719 \\
5000 & 1.0 & 0 & 450 & 3.278000 & 97.768000 \\
4000 & GraMi & 0 & 125 & 28.825000 & 1834.144531 \\
4000 & 1.0 & 0 & 450 & 2.372000 & 97.776000 \\
3500 & GraMi & 0 & 125 & 30.566000 & 1961.636719 \\
3500 & 1.0 & 0 & 450 & 2.372000 & 97.684000 \\
3000 & 1.0 & 0 & 450 & 2.374000 & 97.688000 \\
2500 & 1.0 & 0 & 450 & 2.378000 & 97.684000 \\
2000 & 1.0 & 86 & 3543 & 18.687000 & 97.760000 \\
1500 & 1.0 & 100 & 4550 & 23.805000 & 97.696000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plot/tex/test10.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
2 & GraMi & 19 & 70 & 0.093000 & 54.570312 \\
2 & 1.0 & 9 & 52 & 0.002000 & 5.296000 \\
1 & GraMi & 484 & 2596 & 1.323000 & 466.296875 \\
1 & 1.0 & 313 & 2836 & 0.259000 & 39.920000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plot/tex/wiki-Vote.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
700 & GraMi & 0 & 125 & 0.200000 & 219.093750 \\
700 & 1.0 & 0 & 447 & 0.109000 & 14.028000 \\
600 & GraMi & 0 & 125 & 0.214000 & 223.105469 \\
600 & 1.0 & 0 & 447 & 0.107000 & 14.116000 \\
500 & GraMi & 0 & 125 & 0.199000 & 226.273438 \\
500 & 1.0 & 0 & 447 & 0.108000 & 14.108000 \\
400 & GraMi & 0 & 125 & 1.332000 & 264.191406 \\
400 & 1.0 & 0 & 447 & 0.112000 & 14.056000 \\
300 & GraMi & 91 & 4197 & 46.715000 & 529.179688 \\
300 & 1.0 & 0 & 447 & 0.108000 & 14.052000 \\
200 & 1.0 & 95 & 4089 & 1.053000 & 38.200000 \\
150 & 1.0 & 1084 & 60905 & 69.309000 & 509.864000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plotTable/tex/p2p-Gnutella08.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
100 & GraMi & 125 & 6825 & 84.058000 & 507.472656 \\
100 & 1.0 & 120 & 6016 & 0.725000 & 50.100000 \\
90 & GraMi & 125 & 6825 & 91.347000 & 532.960938 \\
90 & 1.0 & 125 & 6500 & 0.769000 & 53.600000 \\
80 & GraMi & 125 & 6825 & 94.229000 & 503.812500 \\
80 & 1.0 & 125 & 6500 & 0.772000 & 53.604000 \\
70 & GraMi & 125 & 6825 & 98.261000 & 520.980469 \\
70 & 1.0 & 125 & 6500 & 0.778000 & 53.560000 \\
60 & GraMi & 129 & 6932 & 96.405000 & 536.621094 \\
60 & 1.0 & 125 & 6500 & 0.774000 & 53.604000 \\
50 & GraMi & 276 & 14726 & 222.601000 & 648.355469 \\
50 & 1.0 & 139 & 6567 & 0.783000 & 53.616000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plotTable/tex/soc-Epinions1.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
8000 & GraMi & 0 & 125 & 1.079000 & 875.867188 \\
8000 & 1.0 & 0 & 450 & 1.392000 & 61.340000 \\
7000 & GraMi & 0 & 125 & 1.395000 & 812.457031 \\
7000 & 1.0 & 0 & 450 & 1.394000 & 61.304000 \\
6000 & GraMi & 0 & 125 & 1.073000 & 827.636719 \\
6000 & 1.0 & 0 & 450 & 1.398000 & 61.312000 \\
5000 & GraMi & 0 & 125 & 1.009000 & 772.367188 \\
5000 & 1.0 & 0 & 450 & 1.398000 & 61.248000 \\
4000 & GraMi & 0 & 125 & 10.237000 & 955.480469 \\
4000 & 1.0 & 0 & 450 & 1.863000 & 61.352000 \\
3500 & GraMi & 0 & 125 & 10.031000 & 955.500000 \\
3500 & 1.0 & 0 & 450 & 1.390000 & 61.272000 \\
3000 & GraMi & 0 & 125 & 10.275000 & 1024.406250 \\
3000 & 1.0 & 0 & 450 & 1.392000 & 61.340000 \\
2500 & GraMi & 0 & 125 & 10.325000 & 1039.921875 \\
2500 & 1.0 & 0 & 450 & 1.856000 & 61.268000 \\
2000 & GraMi & 0 & 125 & 10.406000 & 993.640625 \\
2000 & 1.0 & 0 & 450 & 1.395000 & 61.304000 \\
1500 & 1.0 & 0 & 450 & 1.393000 & 61.256000 \\
1000 & 1.0 & 100 & 4550 & 13.321000 & 67.520000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plotTable/tex/soc-Slashdot0902.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
8000 & GraMi & 0 & 125 & 27.305000 & 1715.941406 \\
8000 & 1.0 & 0 & 450 & 2.386000 & 97.716000 \\
7000 & GraMi & 0 & 125 & 28.134000 & 1877.316406 \\
7000 & 1.0 & 0 & 450 & 2.388000 & 97.768000 \\
6000 & GraMi & 0 & 125 & 29.227000 & 1590.371094 \\
6000 & 1.0 & 0 & 450 & 2.371000 & 97.676000 \\
5000 & GraMi & 0 & 125 & 29.733000 & 1858.261719 \\
5000 & 1.0 & 0 & 450 & 3.278000 & 97.768000 \\
4000 & GraMi & 0 & 125 & 28.825000 & 1834.144531 \\
4000 & 1.0 & 0 & 450 & 2.372000 & 97.776000 \\
3500 & GraMi & 0 & 125 & 30.566000 & 1961.636719 \\
3500 & 1.0 & 0 & 450 & 2.372000 & 97.684000 \\
3000 & 1.0 & 0 & 450 & 2.374000 & 97.688000 \\
2500 & 1.0 & 0 & 450 & 2.378000 & 97.684000 \\
2000 & 1.0 & 86 & 3543 & 18.687000 & 97.760000 \\
1500 & 1.0 & 100 & 4550 & 23.805000 & 97.696000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plotTable/tex/test10.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
2 & GraMi & 19 & 70 & 0.093000 & 54.570312 \\
2 & 1.0 & 9 & 52 & 0.002000 & 5.296000 \\
1 & GraMi & 484 & 2596 & 1.323000 & 466.296875 \\
1 & 1.0 & 313 & 2836 & 0.259000 & 39.920000 \\
\bottomrule
\end{tabular}


==> results/x399.5m/artifacts/plotTable/tex/wiki-Vote.tex <==
\begin{tabular}{rlrrrr}
\toprule
support & slider & found & searched & timeTaken & memoryUsed \\
\midrule
700 & GraMi & 0 & 125 & 0.200000 & 219.093750 \\
700 & 1.0 & 0 & 447 & 0.109000 & 14.028000 \\
600 & GraMi & 0 & 125 & 0.214000 & 223.105469 \\
600 & 1.0 & 0 & 447 & 0.107000 & 14.116000 \\
500 & GraMi & 0 & 125 & 0.199000 & 226.273438 \\
500 & 1.0 & 0 & 447 & 0.108000 & 14.108000 \\
400 & GraMi & 0 & 125 & 1.332000 & 264.191406 \\
400 & 1.0 & 0 & 447 & 0.112000 & 14.056000 \\
300 & GraMi & 91 & 4197 & 46.715000 & 529.179688 \\
300 & 1.0 & 0 & 447 & 0.108000 & 14.052000 \\
200 & 1.0 & 95 & 4089 & 1.053000 & 38.200000 \\
150 & 1.0 & 1084 & 60905 & 69.309000 & 509.864000 \\
\bottomrule
\end{tabular}


==> tabular/canon.tex <==
\begin{tabular}{|c|c|c|c|}
  \toprule
  mapping & $u_1$ & $u_2$ & $u_3$ \\
  \midrule
  canon \textbf{C} & $b_1$ & $b_3$ & $b_2$ \\
  \bottomrule
\end{tabular}


==> tabular/generator.tex <==
\begin{tabular}{|c|c|c|c|}
  \toprule
  gen & $b_1$ & $b_2$ & $b_3$ \\
  \midrule
  $g_1$ & $b_2$ & $b_1$ & $b_3$ \\
  \bottomrule
\end{tabular}


==> tabular/inverse.tex <==
\begin{tabular}{|c|c|c|c|}
  \toprule
  mapping & $b_1$ & $b_2$ & $b_3$ \\
  \midrule
  inverse canon \textbf{I} & $u_1$ & $u_3$ & $u_2$ \\
  \bottomrule
\end{tabular}


==> tabular/permutation.tex <==
\begin{tabular}{|c|c|c|c|}
  \toprule
  perm & $b_1$ & $b_2$ & $b_3$ \\
  \midrule
  $p_1$ & $b_1$ & $b_2$ & $b_3$ \\ \hline
  $p_2$ & $b_2$ & $b_1$ & $b_3$ \\
  \bottomrule
\end{tabular}


==> tabular/searchedPatterns-0.4.tex <==
\begin{tabular}{llrrr}
    \toprule
     &  & $|S_g|$ & $|S_f|$ & $|S_t|$ \\
    datagraph & support &  &  &  \\
    \midrule
    \multirow[t]{5}{*}{mico} & 9460 & 198 & 0 & 2 \\
     & 9470 & 194 & 0 & 2 \\
     & 9480 & 194 & 0 & 2 \\
     & 9490 & 168 & 0 & 2 \\
     & 9500 & 168 & 0 & 2 \\
    \cline{1-5}
    \multirow[t]{11}{*}{p2p-Gnutella08} & 45 & 363475 & 216170 & 54728 \\
     & 47 & 242253 & 216150 & 53587 \\
     & 49 & 166260 & 162173 & 52648 \\
     & 51 & 122109 & 140546 & 51300 \\
     & 53 & 95081 & 121687 & 49079 \\
     & 55 & 82981 & 104898 & 46220 \\
     & 57 & 75043 & 76129 & 43110 \\
     & 59 & 70910 & 62932 & 38035 \\
     & 61 & 68727 & 52081 & 32573 \\
     & 63 & 67853 & 42497 & 26657 \\
     & 65 & 67025 & 34236 & 20879 \\
    \cline{1-5}
    \multirow[t]{11}{*}{soc-Epinions1} & 1500 & 3573 & 4200 & 1700 \\
     & 1550 & 2375 & 4200 & 1700 \\
     & 1600 & 2375 & 4200 & 1700 \\
     & 1650 & 2375 & 4200 & 1700 \\
     & 1700 & 2375 & 4200 & 1700 \\
     & 1750 & 2375 & 3725 & 1700 \\
     & 1800 & 2375 & 1757 & 1546 \\
     & 1850 & 2375 & 393 & 721 \\
     & 1900 & 2375 & 3 & 29 \\
     & 1950 & 2375 & 0 & 0 \\
     & 2000 & 2375 & 0 & 0 \\
    \cline{1-5}
    \multirow[t]{7}{*}{soc-Slashdot0902} & 2000 & 0 & 5652 & 1700 \\
     & 2250 & 0 & 4200 & 1700 \\
     & 2500 & 23617 & 4200 & 1700 \\
     & 2750 & 2375 & 4200 & 253 \\
     & 3000 & 2375 & 159 & 100 \\
     & 3250 & 2375 & 0 & 100 \\
     & 3500 & 2180 & 0 & 100 \\
    \cline{1-5}
    \multirow[t]{11}{*}{wiki-Vote} & 250 & 0 & 175216 & 0 \\
     & 275 & 0 & 14691 & 0 \\
     & 300 & 0 & 3051 & 14005 \\
     & 325 & 0 & 538 & 1199 \\
     & 350 & 0 & 31 & 67 \\
     & 375 & 220082 & 0 & 0 \\
     & 400 & 5667 & 0 & 0 \\
     & 425 & 2375 & 0 & 0 \\
     & 450 & 2327 & 0 & 0 \\
     & 475 & 2243 & 0 & 0 \\
     & 500 & 1585 & 0 & 0 \\
    \cline{1-5}
    \bottomrule
    \end{tabular}
    
